Linear-Threshold Network Models for Describing and Analyzing Brain Dynamics

Over the past two decades, an increasing array of control-theoretic methods have been used to study the brain as a complex dynamical system and better understand its structure-function relationship. This article provides an overview on one such family of methods, based on the linear-threshold rate (LTR) dynamics, which arises when modeling the spiking activity of neuronal populations and their impact on each other. LTR dynamics exhibit a wide range of behaviors based on network topologies and inputs, including mono- and multi-stability, limit cycles, and chaos, allowing it to be used to model many complex brain processes involving fast and slow inhibition, multiple time and spatial scales, different types of neural behavior, and higher-order interactions. Here we investigate how the versatility of LTR dynamics paired with concepts and tools from systems and control can provide a computational theory for explaining the dynamical mechanisms enabling different brain processes. Specifically, we illustrate stability and stabilization properties of LTR dynamics and how they are related to goal-driven selective attention, multistability and its relationship with declarative memory, and bifurcations and oscillations and their role in modeling seizure dynamics in epilepsy. We conclude with a discussion on additional properties of LTR dynamics and an outlook on other brain processess that for which they might be play a similar role.

==> tex/discussion-conclusions.tex <==
\section{Discussion}\label{sec:discussion}

Our exposition above has illustrated how the basic mechanisms of
goal-driven selective attention, i.e., selective recruitment and
inhibition of neuronal populations based on the particular task, can
be explained arising naturally from the network dynamics.  Feedforward
and feedback play a key role in making possible to inhibit the
task-irrelevant nodes and recruiting the task-relevant ones.  The
control-theoretic perspective we have adopted has been particularly
insightful in unveiling these mechanisms.  In doing so, we have
examined a variety of complex systems, going from a single brain
region modeled as a linear-threshold network, to interconnections of
multiple brain regions giving rise to networks of networks organized
across different topologies. Although we have seen that selective
inhibition and recruitment is achievable for all the considered
topologies, we are interested in analyzing the similarities and
differences for this to happen in terms of structural conditions,
assumptions on the inputs, and the magnitudes of the required control
effort.

% \en{I think this is a too-soon jump into the topic of topology
% comparisons. ``Discussion" section is expected to be more
% general. We can start with some summary of what we have said so far,
% and then move the discussion towards the interesting question that
% naturally arises: similarities and differences between the
% topologies. It's at the same time a bit unusual to have both a
% Discussion section and a Conclusions section. Papers usually have
% one of them or a combination of them under Discussion and
% Conclusions. We can also rename this section to something more
% specific to its content and only have a Conclusions section.}
% {\color{orange} If we move summary from start of conclusions here,
% rename, then have this segment and then future direction
% paragraphs?}  While all three of the topologies considered in
% Section~\ref{sec:topologies} are able to achieve selective
% inhibition and recruitment for the purpose of goal-driven selective
% attention, they do maintain both similarities and differences. Of
% significant interest is these similarities and differences in terms
% of the conditions and control laws required to achieve selective
% inhibition and recruitment.  \marginm{Jorge, you said you would add
% something related to the brain utilizing different neurons for
% different tasks - similar to stuff you have said you use when giving
% talks on this}

\subsection{Selective Inhibition and Recruitment across Topologies} 
In considering the three brain topologies discussed so far, it is
clear that the structure of the hierarchical thalamocortical and
cortical networks maintain strong similarities due to their shared
temporal hierarchies. Meanwhile, the lack of a fixed temporal
hierarchy between the regions in the star-connected network changes
both the form of the conditions for GDSA and the method for proving
the result. The results for the hierarchical networks arise from the
temporal hierarchy, and selective inhibition and recruitment is
achieved as the timescale separation grows large. By contrast, in the
star-connected network without the hierarchy, {\color{blue}the ability to achieve
selective inhibition and recruitment is based only upon the structure and interconnection
of the individual subnetworks.}

It is clear from Theorems~\ref{thrm:cortical_conditions}
and~\ref{thrm:thalamocortical_hierarchy_conditions} that the
conditions for selective inhibition and recruitment in both
hierarchical networks are similar. This is to be expected, given that
the cortical hierarchical network can be seen as a particular case of
the thalamocortical hierarchical network. In particular, the result
for the cortical network can be achieved directly from the
thalamocortical topology by allowing the thalamocortical connections
to equal zero. With the sufficient conditions given in this manner, it
appears more difficult to achieve selective inhibition and recruitment
in the more complex thalamocortical network than in the cortical
one. However, it is important to note that these conditions do not take
into account the inhibitory nature of the connection between the
thalamus and the cortical regions, resulting in a conservative
bounding that leaves room for the existence of tighter conditions
that utilize this feature of thalamocortical communications.

% The hierarchical topologies are both proven using a singular
% perturbation argument based upon the difference between the network
% layer timescales becoming large. The two results have similar
% conditions based upon both the internal dynamics and the
% interconnection pathways, and are sufficient conditions for GES of
% the dynamics of each network layer. It is important to note that for
% networks in which the thalamus is not at the top of the network, the
% sufficient conditions upon the structure of cortical regions above
% the thalamus are more difficult than for the corresponding regions
% in the strictly cortical network. However, for layers below the
% thalamus the conditions are equivalent between the two topologies,
% and if the thalamus is the top layer in the network, the two results
% match for all layers. However, while the sufficient conditions are
% as difficult, or harder, to satisfy for the thalamocortical network,
% we note that the inhibitory nature of the connections between the
% thalamus and the cortical regions are not accounted for in the
% result. Within the nature of the proof mechanisms for GES used
% in~\cite{EN-JC:21-tacII} and~\cite{MM-JC:22}, it is unavoidable to
% ignore this property. However, it does leave room for a potentially
% easier to satisfy condition for GDSA in the thalamocortical network.
% \\

The conditions for GDSA in the star-connected thalamocortical
topology, however, differ significantly from either of the
hierarchical networks. While in the hierarchical networks the
conditions are strongly dependent upon the interconnection properties
between cortical regions, given that these do not exist in the
star-connected network, the conditions are based fully on the internal
dynamics of each network layer. Further, while the achievement of
selective inhibition and recruitment in the hierarchical
thalamocortical network also depends on the interconnection properties
between the thalamus and the cortical regions separately from the
corticothalamic connections, these conditions are paired within the
star-connected network. As such, the assumption that the
corticothalamic feedback is small to avoid pathological
behaviour~\citep{GKK:01} removes conditions upon the thalamocortical
connections in the star-connected network that are needed in the
hierarchical network.

% First, the lack of a hierarchy prevents the use of the singular perturbation proof, and as such the result is proven through a constructive method based upon the network structure. Second, we see that the conditions for selective inhibition and recruitment are dependent mainly upon the internal dynamics of the brain regions, while in the hierarchical networks the interconnection dynamics play a larger role. This follows from the lack of corticocortical connections, and the assumption of small corticothalamic feedback in order to avoid pathological behaviour~\cite{GKK:01}. 

In summary, despite the fact that all three topologies can achieve
selective inhibition and recruitment, as one switches from the
hierarchical networks to the star-connected network, the requirements
change significantly due to the importance of the cortico-cortical
connections and the importance of the thalamocortical connections
within the hierarchical network.

\subsection{Comparison of Control Magnitudes for Selective Inhibition
  and Recruitment}

A second interesting distinction between the three considered
topologies concerns the bounds on the control laws derived in order to
achieve selective inhibition and recruitment. Below we provide the
bounds required for a cortical region in each of the topologies in
order to compare the structural differences across the topologies and
illustrate the benefit of the thalamus with regards to the necessary
control magnitude to achieve selective inhibition and recruitment. In
each of the networks a feedback-feedforward control of the form $\u(t)
= \K\x(t) + \bar{\u}(t)$ is used, and the following equations give
bounds on these quantities. For a cortical layer $\mathcal{N}_i$ in a
hierarchical thalamocortical topology that is below the thalamus, we
have
\begin{align}\label{eq:thalamocortical_hierarchy_controls}
  \B_i^0\K_i &\leq -|\W_{i,i}^{0,\all}| -
  |\W_{i,i+1}^{01}|\bar{\F}_{i+1}|\W_{i+1,i}^{1,\all}|, \notag 
  \\
  \B_i^0\bar{\u}_i(t) &\leq -\W_{i,i-1}^{0,\all}\x_{i-1} -
  \W_{i,T}^{0,\all}\x_T - \c_i^0 -
  |\W_{i,i+1}^{01}|\bar{\F}_{i+1}|\W_{i+1,T}^{1,\all}\x_T +
  \c_{i+1}^1|,
\end{align}
while for a hierarchical cortical layer $\mathcal{N}_i$ we need
\begin{align}\label{eq:cortical_hierarchy_controls}
  \B_i^0 \K_i &\leq -|\W_{i,i}^{0,\all}| -
  |\W_{i,i+1}^{01}|\bar{\F}_{i+1}|\W_{i+1,i}^{1,\all}|, \notag
  \\
  \B_i^0 \bar{\u}_i(t) &\leq -\W_{i,i-1}^{0,\all}\x_{i-1}(t) - \c_i^0,
\end{align}
and for a cortical layer $\mathcal{N}_i$ in the star-connected network
the bounds take the form
\begin{align}\label{eq:star-connected_controls}
  \B_i\K_i &\leq -\W_{i,i}^{0,\all}, \notag
  \\
  \B_i\bar{\u}_i(t) &\leq -\W_{i,T}^{0,\all}\x_T(t) - \c_i^0.
\end{align}
Considering first the feedback control terms, $\B_i^0\K_i$, we note
that they are quite similar across the three topologies. The role of
the feedback is inhibiting the task-irrelevant components of the
internal layer dynamics, which is equivalent across the
topologies. However, in the hierarchical topologies, the feedback
control also accounts for the transfer of information between the
cortical layers, explaining the need for the additional term. This
does not include connections to the thalamus, and as such the
thalamocortical and purely cortical hierarchies maintain an identical
bound on the feedback control. We note that for all three topologies,
the feedback control is based only on local connections (within the
cortex), rather than any thalamocortical connections, which aligns
with the fact that a large amount of feedback control is local, as
discussed in Section~\ref{sec:control_mechanisms_brain_models}.

It is in the feedforward control mechanism that differences in
controls between the topologies is more pronounced. In the
star-connected network, the only connection providing feedforward
control is the connection from the thalamus to the cortical region. In
the hierarchical networks, on the other hand, there is also a bound on
the feedforward control due to the connection from the thalamus and
cortical regions higher in the network. However, in these conditions,
due to the thalamus providing an inhibitory feedforward control to the
cortical regions, it allows for a lower magnitude control signal
(because of the connection from the thalamus increasing the upper
bounds
in~\eqref{eq:thalamocortical_hierarchy_controls},~\eqref{eq:cortical_hierarchy_controls}
and~\eqref{eq:star-connected_controls}). As such, the thalamus
provides a benefit in achieving selective inhibition and recruitment
over strictly cortical networks. This is illustrated in
Figure~\ref{fig:control_magnitude_comparison}, which compares the
required control magnitude to achieve selective inhibition of a
cortical region in a thalamocortical network with the corresponding
cortical network.

% \begin{figure}
%   \includegraphics[scale=0.15]{epsfiles/hierarchical_control_graphon.png}
%   \caption{A depiction of the required control magnitude relative to the magnitude of both corticocortical and thalamocortical connections in the network. For a fixed magnitude of thalamocortical connections there is no clear pattern defining the control magnitude as the corticocortical magnitudes change. However, as the magnitude of the thalamocortical connections increases the overall control magnitude generally decreases.}\label{fig:control_magnitude_graphon}
% \end{figure}
\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.3]{epsfiles/control_magnitude_shaded_error}
  \caption{Illustration of the control magnitude required to
    selectively inhibit the bottom cortical layer averaged over $100$
    random thalamocortical networks and the corresponding cortical
    network in which the thalamus is removed. The shaded regions
    correspond to the error bars.  All of the networks are composed of two cortical regions, each containing three nodes within them. The top cortical layer has one excitatory node while the bottom layer contains only excitatory nodes. The thalamus is composed of two inhibitory nodes. Each thalamocortical and cortical network generated satisfies the assumptions of Theorem~\ref{thrm:cortical_conditions} and
    Theorem~\ref{thrm:thalamocortical_hierarchy_conditions},
    respectively, along with biological sign constraints. The thalamocortical and cortical networks are inhibiting the same set of nodes within the bottom cortical layer in order to make the required control magnitude directly comparable. It is clear
    that the control magnitude required to achieve selective
    inhibition in the thalamocortical networks is significantly lower
    than for the corresponding cortical network without the thalamic
    connections. }\label{fig:control_magnitude_comparison}
\end{figure}

% %
% \marginJC{how did you generate the random networks? How big is $N$,
%   each layer size, etc.? Some details in the caption (for
%   reproducibility) would be necessary. Both types of networks are
%   being driven to the same equilibrium?}
% %

% \en{I don't quite see what the caption says in the figure. I only
% see a brief decrease at the left edge moving rightwards, but then it
% looks pretty flat. Maybe plotting it differently would show the
% pattern? Also, even if one can see the pattern indicated in the
% caption, I can't quite connect it with the paragraph above. Why do
% we need a 3D figure with both thalamocortical and corticocortical
% weighing in it? Shouldn't we have two different figures one for with
% thalamus and one without?}

% \section{Conclusions}\label{sec:conclusions}

% In this work we investigated the use of control-theoretic methods in
% the study of goal-driven selective attention in linear-threshold
% models of the brain. Motivated by the fact that the thalamus has
% been shown to have a significantly larger set of functions than its
% traditional view as a relay station, we consider thalamocortical
% brain networks with topologies based upon different roles of the
% thalamus. In particular, we considered topologies based on two
% classifications of thalamic nuclei, first-order and higher-order,
% which maintain different functions in the brain. First-order nuclei
% provide a topology in which the thalamus acts as a relay of stimuli
% to cortical areas, while the higher-order nuclei modulate
% information being passed between cortical regions.

% We discussed different methodologies for modeling brain networks based upon the varying scales of information and detailed the derivation of firing-rate models in the brain, which we used to model both cortical and thalamocortical networks. These models were then used to detail differences in the ability to achieve goal-driven selective attention in a hierarchical thalamocortical topology, based upon higher-order thalamic nuclei, and a star-connected thalamocortical topology, arising from first-order thalamic nuclei. We found that the ability to achieve selective inhibition and recruitment is based significantly more upon the connections between network regions in the hierarchical network than in the star-connected network, in which the internal dynamics of the network layers play a more prominent role. In addition, while comparing the ability to achieve goal-driven selective attention between a thalamocortical network and a strictly cortical network, we found that the thalamus provides a benefit in terms of the control magnitude required. As the connections from the thalamus to cortical regions operate with using feedforward inhibition, the magnitude of control required decreases in the thalamocortical network compared to the cortical one.
% \en{The structure of these first two paragraphs may benefit from some rewriting where each has a more focused message (and thesis statement at the beginning). Right now they lack a clear flow and structure. Also, I would use ``upon" less frequently :) ``on" works just fine, and sounds less convoluted.}
\subsection{Quantitative Benefit of the Thalamus}\label{sec:quantitative_simulations}


%%% Here provide the simulations on the convergence time relative to variety of parameters.

We have shown that in the hierarchical thalamocortical network we can achieve selective inhibition and recruitment under a set of conditions similar to those for the cortical network. A question of interest that remains is in the benefit of the inclusion of the thalamus in brain networks. Neuroscientific evidence exists for the thalamus allowing the cortex to effectively adjust to rapidly changing behavioural and environmental demands, along with the performance of cognitive functions such as attention and learning~\citep{RN-VK-BD-RB:14}. In this section we investigate simulations of the convergence to equilibrium in selective inhibition and recruitment for hierarchical thalamocortical networks along with their cortical counterparts to illustrate this benefit of the thalamus within our model. In particular we compare how different parameters impact the benefit of the thalamus.

We consider a variety of thalamocortical networks and the corresponding cortical network constructed by removing the connections between the thalamus and cortical regions. In these examples we consider the time it takes for the cortical regions of a network to converge to the selectively inhibited and recruited equilibrium determined by a choice of nodes to be inhibited. These examples are then focused to determine the impact of a variety of network parameters on the convergence time. 
% In particular we consider how the following parameters:


% \marginm{Once all the plots constructed choose which to keep and which to remove based on interest}

% \begin{multicols}{2}
% \begin{itemize}
%     \item Number of layers in the network
%     \item Size of each network layer
%     \item Location of the thalamus in the temporal hierarchy
%     \item Initial distance from equilibrium value
%     \item Ratio of excitatory to inhibitory nodes
% \end{itemize}
% \end{multicols}

We begin by comparing the convergence time as we vary basic system parameters, namely the number of layers in the network and the number of nodes in each network, shown in Figure~\ref{fig:convergence_speed_num_size_layers}. In each of these examples the convergence time is computed and averaged across randomly generated networks and initial conditions while varying the relevant parameters. From Figure~\ref{fig:num_layers} we can see that on average the convergence time for the thalamocortical network is shorter than for the cortical network regardless of the number of layers in the network. Meanwhile Figure~\ref{fig:layer_size} illustrates that at a given number of network layers changing the number of nodes in each layer does not have a significant impact on changing the convergence speed between the thalamocortical and cortical network.

\begin{figure}
  \centering
  \subfigure[]{
  \includegraphics[scale=0.2]{epsfiles/Convergence_Speed/num_layers.png}\label{fig:num_layers}
  }
  % \label{fig:num_layers}
  \subfigure[]{
  \includegraphics[scale=0.2]{epsfiles/Convergence_Speed/layer_size.png}\label{fig:layer_size}
  }
  % \label{fig:size_layers}
  \caption{Comparison of the convergence time for thalamocortical and cortical networks as changing the number of network layers and the size of network layers. (a) Convergence time is compared for networks with a varying number of network layers. For each number of layers $20$ networks are randomly generated and the convergence time to equilibrium is computed and averaged across these networks. The networks are composed of layers with four nodes each, split evenly between excitatory and inhibitory nodes and the initial condition is set a uniform distance from the equilibrium computed to be a fraction of the network threshold value. The thalamus is composed of four inhibitory nodes and the timescale is such that it lies in the middle of the network hierarchy. (b) Convergence time is compared for networks with a varying number of nodes in each layer. For each network layer size $10$ networks are randomly generated and the convergence time is computed and averaged. Each network is composed of $20$ layers and half of the nodes in each layer are excitatory with the remaining inhibitory. The initial condition is set a uniform distance from the equilibrium. The thalamus timescale is set such that it lies in the middle of the network hierarchy.}\label{fig:convergence_speed_num_size_layers}
\end{figure}


Now that we have seen that the thalamus can result in faster convergence to a selectively inhibited and recruited equilibrium we move on to considering thalamocortical networks with varying timescales. These are of interest due to their existence in the brain, as even when considering only the visual thalamus, there exists regions that operate at slow and fast timescales~\citep{ZY-XY-CMH-ZA-NPF-WW-SGB:17}. When varying the thalamus timescale we are considering networks in which the thalamus lies at different points in the temporal hierarchy. For a low timescale the thalamus lies lower in the network and is faster relative to more cortical regions while as the timescale increases the thalamus operates more slowly and moves higher in the network. From Figure~\ref{fig:timescale_varying} we can see that for both fast and slow thalamic timescales the convergence time of the thalamocortical network is lower than that of the strictly cortical network. What is of note is that as the timescale increases and the thalamus becomes slower the margin of improvement decreases. This can be explained by the timescale separation formed in the hierarchy by this increasing timescale. As the timescale continues to increase the thalamus begins to act as a constant relative to the cortical activity, leading to the thalamocortical network essentially becoming a cortical network with a modified constant input, which would then be expected to exhibit behaviour similar to the original cortical network.  Therefore overall it is clear that thalamic regions operating on both fast and slow timescales provide a benefit for network performance of a thalamocortical network compared to a strictly cortical network.

% \begin{figure}
%   \centering
%   \includegraphics[scale=0.25]{epsfiles/Convergence_Speed/timescale_varying.png}
%   \caption{Comparison of the convergence time of thalamocortical and cortical networks with thalamic networks with varying timescales. The convergence time is computed and averaged across $30$ random networks at each thalamic timescale. Each network is composed of $20$ cortical layers of four nodes each, evenly split between excitatory and inhibitory nodes. $250$ thalamic timescales are considered uniformly spread between $0.25$ and $25$ while the cortical regions are linearly spread on the interval $[0.5,5]$. This allows for the consideration of the thalamus at all locations in the hierarchy from below all cortical layers to above. It is clear that all timescales the performance of the thalamocortical network exceeds the strictly cortical network, with the margin of improvement decreasing as the thalamic timescale increases.}\label{fig:timescale_varying}
% \end{figure}


To conclude this section we consider how the thalamus impacts networks with varying ratios of excitatory to inhibitory nodes.  There is significant evidence that inhibition in neural networks is key for selective attention~\citep{AD:13}, with strictly cortical excitatory networks lacking one of the necessary mechanisms required~\citep{ACS-MJM-MAS:16}. Due to the inhibitory nature of the thalamus, the thalamocortical network always maintains the mechanism of inhibitory control that the cortical network can lose with an increase in the proportion of excitatory nodes. As such we expect that as the proportion of excitatory nodes increases the time for convergence of the strictly cortical network will increase while the thalamocortical network will maintain better performance. Figure~\ref{fig:excitatory_ratio} matches these expectations, where we see that in networks with a low proportion of excitatory nodes the thalamocortical networks and cortical networks having essentially identical performance but as the proportion of excitatory nodes increases the thalamocortical network achieves significantly better performance. We note that as the proportion approaches having a fully excitatory network the convergence time drops dramatically, however this follows from the network converging only to zero and the upper threshold, which shortens the convergence time due to decreasing the network equilibrium value.

% \begin{figure}
%   \centering
%   \includegraphics[scale=0.25]{epsfiles/Convergence_Speed/frac_excitatory.png}
%   \caption{Comparison of convergence times of thalamocortical and cortical networks with varying ratio of excitatory to inhibitory nodes. The convergence time is computed and averaged across $30$ random networks composed of $20$ layers with $20$ nodes per layer. The proportion of excitatory nodes rises from a fully inhibitory network to a fully excitatory network (with the exception of the thalamus). For inhibitory networks the performance of the thalamocortical networks and cortical networks is similar. As the number of excitatory nodes increases the performance of the thalamocortical network maintains a similar value while the cortical network is significantly worse. This changes at the high end of the spectrum when the upper bound in the dynamics limits the equilibrium value.}\label{fig:excitatory_ratio}
% \end{figure}



\begin{figure}
  \centering
  \subfigure[]{
  \includegraphics[scale=0.2]{epsfiles/Convergence_Speed/timescale_varying.png}\label{fig:timescale_varying}
  }
  % \label{fig:num_layers}
  \subfigure[]{
  \includegraphics[scale=0.2]{epsfiles/Convergence_Speed/frac_excitatory.png}\label{fig:excitatory_ratio}
  }
  % \label{fig:size_layers}
  \caption{Comparison of the convergence time of thalamocortical and cortical networks with thalamic networks with varying timescales and number of excitatory nodes. a) Convergence time is compared for networks with varying thalamic timescales. The convergence time is computed and averaged across $30$ random networks at each thalamic timescale. Each network is composed of $20$ cortical layers of four nodes each, evenly split between excitatory and inhibitory nodes. $250$ thalamic timescales are considered uniformly spread between $0.25$ and $25$ while the cortical regions are linearly spread on the interval $[0.5,5]$. This allows for the consideration of the thalamus at all locations in the hierarchy from below all cortical layers to above. It is clear that all timescales the performance of the thalamocortical network exceeds the strictly cortical network, with the margin of improvement decreasing as the thalamic timescale increases. b) Convergence time is compared for networks with varying ratio of excitatory to inhibitory nodes. The convergence time is computed and averaged across $30$ random networks composed of $20$ layers with $20$ nodes per layer. The proportion of excitatory nodes rises from a fully inhibitory network to a fully excitatory network (with the exception of the thalamus). For inhibitory networks the performance of the thalamocortical networks and cortical networks is similar. As the number of excitatory nodes increases the performance of the thalamocortical network maintains a similar value while the cortical network is significantly worse. This changes at the high end of the spectrum when the upper bound in the dynamics limits the equilibrium value.}
\end{figure}



\subsection{Conclusions and Avenues for Further Study}

Given the multitude of network structures in the brain, we have set
out to consider the mechanisms for GDSA in multiple different network
topologies. After beginning with a base hierarchical cortical network,
and motivated by the neuroscientific evidence that the thalamus has a
significantly larger set of functions than its traditional view as a
relay station, we have considered different topologies of
thalamocortical brain networks. In each of the network topologies
considered, the thalamus plays a different role. Thalamic nuclei are
broadly divided into two classes, first-order and higher-order,
leading to two different hierarchies. First-order thalamic nuclei
operate as a relay, bringing subcortical stimuli to distinct cortical
areas, resulting in a star-connected topology. Higher-order thalamic
nuclei connect to multiple cortical regions, providing a transthalamic
pathway between them involved in processes such as memory, attention,
and control of cortical
regions~\citep{ASM:15,ASM-SMS-MAS-RGM-RPV-YC:14,LG-SPJ-DEF-MC-MS:05},
and results in a hierarchical network with interconnections between
each of the cortical regions through the thalamus.  After discussing
network models at different information scales within the brain, we
motivated the use of linear-threshold firing rate models for neuronal
dynamics at the mesoscale. We broke down goal-driven selective
attention into two components, selective inhibition and selective
attention, and illustrated how they can be achieved in a single region
brain model. Using the insights gained, we then expanded upon the
mechanics of goal-driven selective attention to larger brain networks
of networks.

Our considered topologies and obtained results on the roles of the
thalamus in GDSA is by no means comprehensive and there is still the
potential that the thalamus plays a larger role in GDSA than what has
been articulated here. While constructing topologies based on the
first- or higher-order roles of the thalamus is an important factor in
modeling these networks, more elaborate models can be constructed
based on further details of the thalamus circuitry and specific
functions (e.g. in working memory).
% %
% \marginJC{Missing info after ``e.g.,'' here }
% %
These detailed models can contain additional properties of the
thalamus beyond the inspiration here driven by its impact on cortical
regions through feedforward inhibition. As noted earlier, however, our
ability to illustrate an improvement in control magnitude using the
feedforward inhibition of the thalamus and the sufficient conditions
on which this improvement relies where obtained without taking any
advantage of the inhibitory nature of thalamic feedforward
connections. Therefore, even within thalamocortical models at the
level of detail considered here, it is possible that the thalamus
plays a larger role than shown.
% Constructing detailed models to create thalamocortical network
% topologies relevant to a specific task in which the thalamus is
% involved, such as working memory, we could find that the thalamus
% plays an even more significant role, potentially to the point in
% which GDSA is not possible without thalamocortical connections.
The thalamus has been shown to contribute to and even orchestrate a
large array of brain functions beyond GDSA, including sleep and
consciousness~\citep{TCG-MB-CGH-ARA:18},
oscillations~\citep{MM-WJE-NP:15}, learning and
decision-making~\citep{ASM:15,ZO-HF-ASM:18}, and bottom-up
(stimulus-driven) selective
attention~\citep{RDW-LIS-TJD-MN-KD-MMH:15}.
% \en{???~\cite{???}, what comes to my mind is sleep and memory
% consolidation, consciousness, oscillations, bottom-up
% (stimulus-driven) selective attention, reward processing and
% reinforcement learning}.
Nevertheless, despite the prevalent use of computational network
models, including thalamic regions, for the study of these functions,
see e.g.,~\cite{KH-MAB-WBL-MD:17,ND-RDW:19,TDW-JK-TDJ-TEN-ABS-LFB:15},
applications of network control theory are lacking outside of the role
of the thalamus as a relay within the brain.
%  which has led to the control-theoretic models of remote
%  synchronization. 
This highlights the various avenues that exist for future study of the
various roles of the thalamus from a controls perspective, both in
further understanding of GDSA and beyond.
% While we have investigated the thalamus and its role in a
% control-theoretic modeling approach to GDSA, in the neuroscience
% literature it has been shown the thalamus has a role in many more
% applications within the set of brain functions.  However, outside of
% its role as a relay within the brain, which led to control-theoretic
% models of remote synchronization in thalamocortical networks, the
% application of network theory to models of the thalamus is
% lacking. While works utilizing computation brain models, including
% network models, exist for brain functions that involve the thalamus,
% such as perception, creativity, and conscious motor action, there is
% minimal focus upon the role of the thalamus, particularly within
% those using network models. As such, there are many avenues for
% future study of thalamocortical networks using network models, both
% in further exploring GDSA, or in one of the many other functions of
% the thalamus.


==> tex/introduction.tex <==
\section{Introduction}
The brain is one of the most complex dynamical systems known to exist,
composed of billions of interconnected neurons and involved in
countless cognitive and physical functions in the body. With such a
vital role, creating computational models of the brain to explain how
these functions work is critical.
% It is of such interest that reverse engineering the brain is one of
% the National Academy of Engineering's $14$ grand challenges for the
% $21^{\text{st}}$ century.
The complexity that arises from the interplay between neuronal
dynamics, multiple temporal and spatial scales, and the intricate
interconnection and rich topological structure observed in the brain
makes the use of system-theoretic techniques a natural choice to
analyze and understand such computational models.  A number of works,
see
e.g.,~\citep{SJS:12,SG-FP-MC-QKT-ABY-AEK-JDM-JMV-MBM-STG-DSB:15,MSM-NJC:20,SC-MYL-JJC-MBW-JDK-KS-PLP-ENB:13,EN-JC:21-tacI,EN-JC:21-tacII,PS-EN-JZK-HJ-DZ-CB-FP-GJP-DSB:20,GD-TOL-JD-AF-RF:15},
% %
% \marginJC{Is this all the people we want to cite? How about something
%   by ShiNung Ching, Rodolphe Sepulchre, Erfan,...?}
% %
have recently advocated for this combination between control and
neuroscience.  This paper contributes to this body of work by studying
thalamocortical networks with different topologies achieving selective
recruitment and inhibition in the context of goal-driven selective attention.
% \en{reads very well, but a bit too direct in conveying a message
% that perhaps no one would argue against. Really subtle point
% though. can be potentially shrunk a bit. Also, the last sentence
% doesn't ``end" the paragraph, i.e., it's not a ``concluding"
% sentence for the paragraph. You can maybe say something about what
% this paper is going to do in the little context you created.}


Since the brain is composed of systems performing various functions,
it is unrealistic to expect one single model to be able to
accurately describe all phenomena.
%  and, therefore, it is important to
% develop and study a variety of models in the brain. 
In particular, since distinct functions utilize
different areas in the brain, it is of interest to study
a variety of model architectures to explain these phenomena.
% %
% \marginJC{Re-read the intro carefully making sure you avoid
%   repeating the same word in the same sentence (sometimes, 3
%   times!), ideally avoiding in consecutive sentences too.}
% %
A majority of the literature on brain networks studies the cortex and
cortical networks~\citep{GTE-CK-NKL-SP:13,QL-AU-BH:17,MK-RN-FG-MK-YI-TA-MS:21,JC-UH-CJH:15} due to its role in higher-level processes in the
brain, such as memory, perception, and voluntary motor
movement~\citep{MB-BC-MAP:20}.
% %
% \marginJC{The ref is for the high-level processes or for ``lit on
%   brain networks''? In any case, 1 ref seems too little for a
%   reference to a majority of the literature.}
%   \marginm{Was playing both, but added different and more references for studies on cortex}
% %
%
% \en{cortex is in fact a very tiny portion of the brain. cerebellum
% alone has about 60\% of brain neurons. cortex is really loved
% because it is the most recently developed (and thus more
% ``advanced") part of mammalian (particularly primate) brain.}
 %
However, most cortical regions have inputs from subcortical areas,
including the thalamus, that play critical roles in the many functions
undertaken by the cortex~\citep{SMS-RWG:06}. This includes almost all
functions that involve sensory input, as one of the roles of the
thalamus is the relay of sensory inputs to the
cortex~\citep{KH-MAB-WBL-MD:17}. In addition, it has also been found
that for almost all connections between cortical regions, there
exists a transthalamic parallel pathway~\citep{SMS:12}. As such, it is
of significant interest to study thalamocortical networks containing
these parallel pathways in addition to the more commonly analyzed
strictly cortical networks.


We note that with regions such as the thalamus having multiple roles,
the connections between the subregions involved in each role is not
necessarily the same. As such, even within the class of
thalamocortical networks, it is important to consider different
network topologies. In this work, we focus on the role of the thalamus
in brain networks and study two different topologies based on
different roles it plays. First, as a relay of sensory inputs to
multiple areas with the cortex, it is natural to consider a
star-connected topology. Second, motivated by its role as a parallel
pathway for information transfer between cortical regions
  and the well-known hierarchical structure of the
brain~\citep{NT:50,ARL:70,DJF-DCEV:91}, we also consider a
thalamocortical hierarchical topology. In order to delineate the
specific roles of the thalamus in the latter, we further compare and
contrast this thalamocortical hierarchy with a purely cortical
hierarchical topology devoid of the thalamus~\citep{EN-JC:21-tacI,EN-JC:21-tacII,MM-JC:22}.


% Regardless of the function of a given brain network, the amount of information input into the system contains both information relevant to the current task, as well as a variety of additional information, or distractions. The process of active selection of the relevant input information to process, while concurrently inhibiting the effects of the distractions is known as goal-driven selective attention (GDSA) and is vital for the function of the brain. In this work we investigate the mechanisms of GDSA in the variety of brain topologies discussed above. 

% %
% \marginJC{As always, avoid future tense, use present instead. Also,
%   ``we are unable'' sounds negative, where in reality there is nothing
% wrong with it -- and pretending otherwise would be foolish. Reword to
% not focus it on ``inability'', but instead on the sheer complexity of
% the biological entity.}
% %

Even while limited to thalamocortical networks with the topologies
described above, due to the complexity and quantity of brain functions associated with the thalamus, it is unrealistic to accurately explain each of these functions with a single model. As such, we further
restrict our focus in studying these networks to a single task
relevant to all of the topologies. In particular, we investigate a central phenomena underlying the brain's broad
ability to process sensory information and make sense of the world known as \emph{goal-driven
  selective attention} (GDSA). As all of the brain's functions are
based upon responses to the environment around it, GDSA is a
fundamental building block for all other functions of the brain.


At any point in time the brain is receiving a constant flow of
sensory information and, for any given task, only a subset of this
information is relevant. GDSA is the process in which the brain
actively determines which subset of the information is relevant for
the current task in order to process it, while simultaneously suppressing
the remaining irrelevant inputs. These two components are
referred to as \emph{selective recruitment} and \emph{selective
  inhibition}, respectively. Some of the most obvious examples of GDSA
include selective vision in busy visual
fields, selective listening in a noisy environment, and selective
smell. However, GDSA extends well beyond just sensory processing. For instance, GDSA also becomes fundamental in working memory in order to select related relevant information
from internal representations~\citep{FvE-AGB-ACN:20,MMC-JDG-NBTB:11,ACN-MGS:19}.


Given its importance, %in allowing for proper function of the brain, 
GDSA has been the subject of significant research in the
neuroscience community,
see e.g.,~\citep{JS:90,AMT:69,ECC:53,RD-JD:95,LI-CK:01,BCM:93,MAP-GMD-SK:04},
among many more. A variety of experimental methods have been used to better elucidate the various aspects of GDSA,
including working memory tasks~\citep{FvE-AJQ-MWW-ACN:18}, auditory
discrimination tasks~\citep{ECC:53}, and visual searching
tasks~\citep{MAP-GMD-SK:04}. Nevertheless, despite this significant body of research,
it was only until our recent work~\citep{EN-JC:21-tacI,EN-JC:21-tacII} where a dynamical computational understanding of GDSA
from a model-based perspective was established. 
\marginm{GDSA and the thalamus - potentially move}

{\color{blue}
  While~\citep{EN-JC:21-tacI,EN-JC:21-tacII} provides a model-based perspective for GDSA for cortical networks it does not consider the important role of the thalamus in selective attention. In fact, the thalamus is inextricably linked with the cortical processes involved in selective attention~\citep{JN:95}. With GDSA the role of the thalamus is to mediate information transfer, both between cortical regions and between subcortical regions and the cortex. First, the thalamus `gates' information flow to a given region of the cortex, allowing for the the relevant information for the target of selective attention to reach the region while preventing other irrelevant information~\citep{JN:95}. Second, the thalamus modulates the flow of information between the cortical regions. Rather than directly selecting the relevant information for the desired target, it does so as a gain operator on the traveling information, enhancing the relevant information traveling between cortical regions and inhibiting the irrelevant information~\citep{DL-MC-VB:92}. This work reviews and extends upon the results
of~\citep{EN-JC:21-tacI,EN-JC:21-tacII} while considering the role of the thalamus in GDSA.


}
% \en{This section is too brief and appears out of the blue. Note that we spent two rather long paragraphs just to talk about thalamus (which is all ok), but then only a short one to discuss a very important aspect of this paper: focusing on a very specific task out of the numerous tasks the brain does and we even mention above. I think we need at least two paragraphs here. One that is aimed at narrowing our focus on GDSA, in which we warm up the reader by saying that we can't study everything that the brain does so we are going to be more focused. And we focus on a very important phenomena that underlies the brain's ability to make sense of the world and therefore anything else that the brain does. This can just end the first paragraph. Then we can move to the second paragraph (maybe with a third, if necessary) and introduce GDSA much more comprehensively. What it is, how general it is (going even beyond sensory processing to working memory and perhaps anywhere that the brain has to allocate limited neuronal resources to competing streams of information), what people in neuroscience have done to study it, etc.}

\begin{myblock}{The Thalamus: More Than a Relay
    Station}\label{box:thalamus}
  % \subsection*{The Thalamus: More Than a Relay
  % Station}\label{box:thalamus}
  The thalamus is a component of many different brain networks and
  thus plays a role in a large number of functions. Traditionally, the
  thalamus has been considered primarily as being a sensory relay to
  the cortex, playing minimal other functional
  roles~\citep{MW-SDV:19}. Despite being known since the late
  $19^{\text{th}}$ century to have additional functions such as a
  role in memory loss~\citep{HG:96}, up until recently the majority of
  the research into thalamic function has studied its function as a
  sensory relay~\citep{SMS-RWG:06,EA-TO:15,YBS-SK:11}.  This view was
  gradually changed by several works, including the pioneering
  work~\citep{SMS-RWG:96}, establishing the thalamus as an
  heterogeneous structure only a small portion of whose nuclei play
  the role of a sensory relay. Following this work, research has shown
  the thalamus plays a role in learning and memory~\citep{ASM:15},
  attention, impulse control and
  decision-making~\citep{ASM-SMS-MAS-RGM-RPV-YC:14,FA-VF-ARM-EJK-EC-WM:18},
  and feedforward inhibitory control of cortical
  regions~\citep{ASM-SMS-MAS-RGM-RPV-YC:14,JMA-HAS:15,LG-SPJ-DEF-MC-MS:05,MMH-LA-16}.
  
  
  Thalamic nuclei can be broadly divided into two categories depending
  on their role in these applications. Nuclei involved mainly in the
  role of the thalamus as a sensory relay are known as
  \emph{first-order} and receive their input from other subcortical
  structures. The thalamic nuclei involved in the variety of other
  brain functions associated with the thalamus are referred to as \emph{higher-order} and receive their
  inputs from varying cortical regions~\citep{SMS:12}. The higher-order
  nuclei are then able to directly elicit activity in cortical regions
  based upon modulation of the latter's input signals, leading to the
  contribution of the thalamus to the brain functions above. With
  these divided roles in thalamic function, it is relevant to
  construct separate models for explaining their functions in brain
  networks.
  

  When the thalamus interacts with cortical regions, it does so
  through feedforward inhibitory
  control~\citep{JMA-HAS:15,LG-SPJ-DEF-MC-MS:05,SJC-TJL-BWC:07}. As
  such, when studying thalamocortical networks, the models must take
  into account that connections from the thalamus to cortical regions
  are inhibitory, while returning connections could be either
  excitatory or inhibitory. In the context of modeling the brain from
  a control-theoretic perspective, the thalamus provides an
  exciting avenue of study due to its role as an internal
  controller. While maintaining its own dynamics, it concurrently
  works to control the cortical dynamics by modulating and
  transferring information between cortical regions in parallel to the
  cortico-cortical transmissions.
 \end{myblock}

\subsection*{Outline}
The paper is organized as follows. In
Section~\ref{sec:brain_modeling}, we discuss methods of modeling the
brain, focusing on firing rate models and mechanisms for control in
the brain. Section~\ref{sec:GDSA_single_network} explores the mathematical phrasing of selective inhibition and recruitment before looking at GDSA within a single brain region. In
Section~\ref{sec:topologies}, we discuss the construction of networks
of brain regions and GDSA in thalamocortical networks with different
topologies.  Finally, in Section~\ref{sec:discussion}, we discuss
similarities and differences between the results across the different
topologies before providing concluding remarks and potential further
avenues of study.
% %
% \marginJC{Repeated Section 5 in the same sentence. Give a careful read
% to the whole paper to smooth the presentation: the exposition would
% benefit from some polishing with a global perspective (to correct for
% small inconsistencies caused by fixing things here and there at
% different times).}
% %


==> tex/selective.tex <==
\section{Goal-driven Selective Attention in a Single Brain Region} \label{sec:GDSA_single_network}%in a Linear-Threshold Model for a Brain Network}

% \en{I think we need to begin with some motivation here. Essentially,
% why should the reader care what model we consider here, etc.? What
% overall interesting question we will answer by doing this? Then we
% can get to the specifics of what model type we'll be using, etc. If
% you have said this before, you may just say something like ``Recall
% our guiding question of ... and, in particular, its reliance on our
% understanding of ... ".}
As we have outlined in the introduction, our guiding question is that
of understanding, from a model-based perspective, the phenomenon of
goal-driven selective attention. This brain function strongly relies
on the ability to selectively recruit and inhibit neuronal
populations. Here, we analyze how both of these can be explained in
the dynamical context of firing rate models introduced in
Section~\ref{sec:brain_modeling}.

We consider a brain region composed of $n$ nodes, with each node
representing a population of either excitatory or inhibitory neurons,
and governed according to the linear-threshold dynamics
in~\eqref{eq:network_lin_threshold dynamics}.  The network structure,
cf.  Figure~\ref{fig:single_brain_layer}, is encoded by the synaptic
weight matrix $\W$. Here we focus on a single brain network before
addressing in the next section more complex scenarios involving
networks of networks modeling the interconnection of multiple brain
regions.  We begin by formalizing the problem of selective inhibition
and recruitment within the framework of linear-threshold firing rate
dynamics.

\subsection{Mathematical Phrasing of Selective Inhibition and Recruitment}\label{sec:math-def}
Selective inhibition and recruitment is the process of identifying
task-irrelevant and task-relevant stimuli, and suppressing the
task-irrelevant ones while processing the task-relevant ones. Since
different stimuli are, to a first approximation, processed by distinct
populations of neurons~\citep{RD-JD:95,JM-RD:85,BCM:93,NL:05} (a fact
closely related to the sparseness of the neural
code, see~\cite{FP:03,MI-AR-DK-TR-JMR:17}), this can be rephrased as
inhibiting the populations of neurons associated with the
task-irrelevant stimuli and recruiting the populations associated with
task-relevant stimuli. As such, we partition both the state variables
$\x \in \R^n$ and the synaptic weight matrix $\W$ based upon the
task-irrelevant and task-relevant nodes, as follows
\begin{align}\label{eq:partition_state_variables_and_matrix}
  \x(t) = \begin{bmatrix}
    \x^0(t) \\
    \x^1(t)
  \end{bmatrix} \qquad \W = \begin{bmatrix}
    \W^{00} & \W^{01} \\
    \W^{10} & \W^{11}
  \end{bmatrix}.
\end{align} 
Then, inhibiting the task-irrelevant stimuli corresponds to driving
$\x^0$ to $\zero$, whereas processing the task-relevant stimuli
corresponds to driving $\x^1$ to a desired attractor $\x^1_*$. While
the ensuing framework is generalizable to arbitrary attractors, for
simplicity of exposition, in our treatment we consider $\x^1_*$ to be
a desired equilibrium. Accordingly, we also partition the input
$\d(t)$ from~\eqref{eq:network_lin_threshold dynamics} as
\begin{align*}
	\d(t) = \B\u(t) + \tilde{\d}(t),
\end{align*}
where
\begin{align*}
  \B = \begin{bmatrix}
    \B^0 \\
    \zero
  \end{bmatrix} \qquad \tilde{\d}(t) = \begin{bmatrix}
    \zero \\ \tilde{\d}^1(t)
  \end{bmatrix},
\end{align*}
resulting in the dynamics
\begin{align}\label{eq:full_lin_thresh_dynamics_for_selective_inhibition}
  \tau{\begin{bmatrix}
      \dot\x^0(t) \\
      \dot\x^1(t)
    \end{bmatrix}} = -\begin{bmatrix}
    \x^0(t) \\
    \x^1(t)
  \end{bmatrix} + \left[\begin{bmatrix}
      \W^{00} & \W^{01} \\
      \W^{10} & \W^{11}
    \end{bmatrix}\begin{bmatrix}
      \x^0(t) \\
      \x^1(t)
    \end{bmatrix} + \begin{bmatrix}
      \B^0 \\
      \zero
    \end{bmatrix}\u(t) + \begin{bmatrix}
      \zero \\ \tilde{\d}^1(t)
    \end{bmatrix} \right]_\zero^\m.
\end{align}
This decomposition allows us to separate the inhibition of the
task-irrelevant populations from the recruitment of the task-relevant
populations. The term $\B^0\u(t)$ allows for the inhibition of the
task-irrelevant populations through either an external control source
or connections with another controlling neuron population. Meanwhile,
the term $\tilde{\d}^1(t)$ allows for the recruitment of the
task-relevant populations by representing the information pathways
between different brain regions along with any additional unmodeled
activity impacting the equilibrium to which the task-relevant
components are recruited.

Figure~\ref{fig:inhibition_recruitment_with_inputs} illustrates the
discussion above.
\begin{figure}
\centering
  \includegraphics[scale=0.5]{epsfiles/selectively_inhibited_w_labels}
  \caption{Brain region divided into task-irrelevant (grey) and
    task-relevant (red and blue) neuron populations. The
    task-irrelevant nodes make up $\x^0$ in the partition of the
    state, while the task-relevant nodes form $\x^1$. The control
    input $\u(t)$ is used to selectively inhibit the task-irrelevant
    populations, while the input $\tilde{\d}^1$ recruits the
    task-relevant populations to an
    equilibrium.}\label{fig:inhibition_recruitment_with_inputs}
\end{figure}

With these decompositions in place, the problem of selective
inhibition and recruitment of the network can now be formulated
mathematically as follows: under what conditions on the network
structure can we find control $\u(t)$ such that the network dynamics
are stabilizable to $(\zero,\x_1^*)$?


\subsection{Selective Inhibition and Recruitment of a Linear-Threshold Brain Network}\label{sec:inh-rec-lt}
The ability to achieve selective inhibition and recruitment depends on
the stabilizability of the network through feedforward and feedback
control mechanisms.  Understanding stabilizability, in turn, requires
understanding the stability properties of the dynamics, and how the
interconnection structure of the network affects it.  Our ensuing
discussion tackles this point.

\subsubsection{Stability of Linear-Threshold Networks as a Function of
  Interconnection Structure}\label{sec:stability-conditions}
For simplicity, we assume that the input term is constant, $\d(t) =
\d$, before generalizing the discussion to time-varying $\d(t)$
subsequently. The stability properties of the dynamics are closely
related to its network structure, which in the linear-threshold brain
model is encoded into the synaptic connectivity matrix $\W$. As such,
we introduce the following notions  of matrix classes.

\begin{definition}\label{def:matrix_classes}
  A matrix $\W \in \R^{n \times n}$ is
  \begin{itemize}
  \item \emph{absolutely Schur stable} if $\rho(|\W|) < 1$ where $\rho(\cdot)$ is the spectral radius;
  \item \emph{totally $\mathcal{L}$-stable} ($\W \in \mathcal{L}$) if
    there exists $\bf{P} = \bf{P}^\top > \zero$ such that for all
    $\sigma \in \{0,1\}^n$
    \begin{align*}
      (-\eye + \W^\top \Sigma)\bf{P} + \bf{P}(-\eye + \Sigma \W) < 0,
    \end{align*}
    where $\Sigma = \mathrm{diag}(\sigma)$;
  \item \emph{totally Hurwitz} ($\W \in \mathcal{H}$) if all its
    principal submatrices are Hurwitz;
  \item a \emph{P-matrix} ($\W \in \mathcal{P}$) if all its principal
    minors are positive.
  \end{itemize}
\end{definition}

We note that these matrix classes admit a variety of inclusions, as
shown in Figure~\ref{fig:matrix_class_inclusions}.
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{epsfiles/venn.pdf}
  \caption{Inclusions satisfied by the different matrix classes in
    Definition~\ref{def:matrix_classes}.}\label{fig:matrix_class_inclusions}
\end{figure}

Using these matrix classes, we can provide conditions for both the
existence and uniqueness of equilibria (EUE) and global exponential
stability (GES) of the dynamics
\begin{align*}
  \tau\dot{\x} = -\x + [\W\x + \d]_\zero^\m.
\end{align*}
In particular, following~\cite{EN-JC:21-tacI}, the dynamics have a
unique equilibrium point if and only if $\eye-\W \in \mathcal{P}$, are
locally asymptotically stable if and only if $-\eye + \W \in
\mathcal{H}$, and are GES if $\W \in
\mathcal{L}$. Further,~\cite{EN-JC:21-tacI} conjectures that $-\eye +
\W \in \mathcal{H}$ is necessary and sufficient for GES. One challenge
with using these results, however, is that determining that matrices
are P-matrices or totally Hurwitz is computationally challenging,
especially as the scale of the network increases. As such, the
inclusions in the matrix classes from
Figure~\ref{fig:matrix_class_inclusions} take on importance as they
can be used to construct more conservative conditions (such as the
conditions based on the spectral radius and norm of $\W$) for EUE and
GES that are computationally tractable.

\subsubsection{Achieving Selective Inhibition and Recruitment through
  Feedforward and Feedback}
Given the importance of feedforward and feedback control for the
brain, cf. Section~\ref{sec:control_mechanisms_brain_models}, we
consider achieving selective inhibition and recruitment using both
mechanisms. Here, we characterize first each mechanism separately and
later discuss the advantages of the combinations thereof.

We begin by considering feedforward inhibition.
% We will denote the brain region we are modeling by $\mathcal{N}$
% \en{can we just remove $\mathcal{N}$ from here and the foregoing
% theorems/discussions? I don't see its utility when we have only one
% network}, and let it be governed by the dynamics
% in~\eqref{eq:full_lin_thresh_dynamics_for_selective_inhibition}.
In this case, the brain region under consideration is being inhibited
by a separate (not explicitly modeled here) brain region to an
activity/inactivity pattern of its choice through the control
input~$\u(t)$. Since the linear-threshold activation function is
unaffected by excessive inhibition due to its thresholding at zero,
selective inhibition through feedforward inhibition is possible by
using a sufficiently strong inhibitory input. Utilizing this, and the
conditions for stability of a linear-threshold dynamics described in
Section~\ref{sec:stability-conditions}, we can formalize the following
conditions.

\begin{theorem}\longthmtitle{Selective Inhibition and Recruitment
    through Feedforward Inhibition~\citep[Theorem
    V.2]{EN-JC:21-tacI}}\label{thm:feedforward_selective_inhib}
  Consider a brain region modeled with the linear-threshold
  dynamics in~\eqref{eq:full_lin_thresh_dynamics_for_selective_inhibition}. Suppose
  that $\dim(\u(t)) \geq \dim(\x^0)$ and that
  \begin{align*}
    \range([\W^{00} \ \ \W^{01}]) \subseteq \range(\B^0).
  \end{align*}
  Then, for any constant $\tilde{\d}^1$,
  % % 
  % \marginJC{Why $\tilde{\d}^1$ and not the simpler $\d^1$?}
  % \marginm{To maintain consistency with prior subsection. Intuitively $\d^1$ would mean instead $\B^1\u(t) + \tilde{\d}^1$}
  % % 
  there exists a constant feedforward control input $\u(t) = \bar{\u}$
% %
% \marginJC{Should we use $\bar{\u}$ instead of $\u$ to keep it
%   consistent with the notation we use in Section 4?}
% %
 that
  stabilizes the dynamics to the unique equilibrium of the form
  $(\zero,\x^*)$
  % $\mathcal{N}$ can be selectively inhibited and recruited
  % \en{[``can be selectively inhibited and recruited" is too vague I
  % think, both because we have a Theorem environment and also because
  % I think we defined what we mean by this a while ago in the
  % paper. the same applies to the next theorem as well.]}
  if and only if $\W^{11}$ is such that the internal dynamics
  \begin{align*}
    \tau\dot{\x}^1 = -\x^1 + [\W^{11}\x^1 + \tilde{\d}^1]_\zero^{\m^1}
  \end{align*}
  is GES to a unique equilibrium.
\end{theorem}

We discuss the interpretation of the conditions of this result at the
end of the section, in parallel with the feedback inhibition case.  We
note that in Theorem~\ref{thm:feedforward_selective_inhib} the
potential for selective inhibition and recruitment is predicated on
the stability of the uncontrolled portion of the dynamics. This
illustrates that the properties required for selective inhibition and
selective recruitment can be fully separated. The ability for
selective inhibition is based upon the dynamics for the
task-irrelevant nodes, while selective recruitment is based upon only
the dynamics of the task-relevant nodes, with no intersection. In a
similar fashion, for selective inhibition and recruitment using
feedback inhibition, the conditions are dependent only upon the
structure of the task-relevant component of the synaptic weight
matrix, and are given as follows.

% \en{I think it's good to describe somewhere in this discussion the
% role of the auxiliary conditions in these two theorems (on the
% number of channels in $\u$ and the range condition). We can even
% mention that the condition on the number of channels in $\u$ does
% not appear in the feedback case as at least an interesting
% observations, and perhaps more if we have more insights on it
% (nothing that I can immediately think of)}

\begin{theorem}\longthmtitle{Selective Inhibition and Recruitment
    through Feedback Inhibition~\citep[Theorem
    V.3]{EN-JC:21-tacI}}\label{thrm:feedback_selective_inhib}
  Consider a brain region modeled with linear-threshold
  dynamics in~\eqref{eq:full_lin_thresh_dynamics_for_selective_inhibition}. Let
  the input $\u(t)$ be given by the linear feedback
  \begin{align*}
    \u(t) = \K\x(t),
  \end{align*}
  where $\K$ is a constant control gain and suppose $\dim(\u(t)) \geq \dim(\x^0)$. Further, assume that
  $\range([\W^{00} \ \ \W^{01}]) \subseteq \range(\B^0)$. Then, there
  almost always\footnote{That is, the set of allowable matrix pairs $(\W,\B)$ for which no satisfactory matrix $\K$ exists, is of measure zero. }
  % % 
  % \marginJC{What does ``almost always'' mean here? Like generically?
  %   In what sense (space of all allowable matrices?).  We need to explain it,
  %   here in a footnote, or after the statement.}
  % % 
  exists a $\K$ such that
  \begin{enumerate}[i)]
  \item $\eye - (\W+\B\K) \in \mathcal{P}$ if and only if $\eye -
    \W^{11} \in \mathcal{P}$;
  \item $-\eye + (\W+\B\K) \in \mathcal{H}$ if and only if
    $-\eye+\W^{11} \in \mathcal{H}$;
  \item $\W+\B\K \in \mathcal{L}$ if and only if $\W^{11} \in \mathcal{L}$;
  \item $\rho(|\W+\B\K|) < 1$ if and only if $\rho(|\W^{11}|) < 1$;
  \item $\norm{\W+\B\K} < 1$ if and only if $\norm{[\W^{10}~\W^{11}]}
    < 1$.
  \end{enumerate}
\end{theorem}

% \en{I'm a bit skeptical about the last statement of the theorem. for
% example, if $\eye - \W^{11} \in \mathcal{P}$ but the task-relevant
% subnetwork is not totally Hurwitz (and hence the unique equilibrium
% is unstable), then we won't have selective inhibition and
% recruitment, right?}

The interpretation of each of the results in
Theorem~\ref{thrm:feedback_selective_inhib} is as follows.  First,
recalling that selective inhibition and recruitment occurs when the
system is stabilizable to a unique equilibrium $(\zero,\x^*)$,
Theorem~\ref{thrm:feedback_selective_inhib}$i)$ guarantees the
existence and uniqueness of the equilibrium $\x^*$ for the
task-relevant components. However, this condition does not guarantee
the equilibrium is stable, so it is not sufficient for selective
inhibition and
recruitment. Theorem~\ref{thrm:feedback_selective_inhib}$ii)$ then
guarantees local asymptotic stability (and potentially GES) of the
equilibrium point $\x^*$. The remaining conditions utilize the matrix
inclusions given in Figure~\ref{fig:matrix_class_inclusions} to
provide sufficient conditions for stabilizability of the task-relevant
conditions to the
equilibrium~$\x^*$. Theorem~\ref{thm:feedforward_selective_inhib}$iii)$
guarantees GES of the task-relevant components of the dynamics to
$\x^*$, thus providing a sufficient condition, when combined with the
assumptions of the theorem, that selective inhibition and recruitment
is achievable through stabilization to $(\zero,\x^*)$. Condition $iv)$
does not guarantee GES, as the matrix class $\rho(|\cdot|) < 1$ is not
a subset of the class of $\mathcal{L}$-stable matrices, but it is more
computationally tractable and does guarantee local asymptotic
stability. Finally, Theorem~\ref{thrm:feedback_selective_inhib}$v)$ is
computationally tractable, and is sufficient for guaranteeing GES of
the equilibrium $\x^*$, allowing for stabilizability to
$(\zero,\x^*)$.

% \en{Since most people don't read linearly or carefully enough, I
% think it's useful to remind the reader why we care about the
% conditions in the theorem. Like a brief reminder that item (i) is a
% necessary and sufficient condition for EUE, etc. In general, I think
% these two results by themselves lack a strong intuitition. They are
% supposed to be just parallels of each other while in reality they
% give necessary and sufficient conditions for slightly different
% things. So I think spending some time clarifying what each if/then
% condition means in each of them, how similar they are, and how
% different they are will be very helpful.}

To conclude this section, we discuss the assumptions in
Theorems~\ref{thm:feedforward_selective_inhib}
and~\ref{thrm:feedback_selective_inhib}. Both the feedforward and
feedback case require an assumption on the relationship between the
range of the task-irrelevant component of the synaptic weight matrix
and the task-irrelevant component of the inhibitory control
matrix~$\B^0$.  In both results, the purpose of this condition is to
guarantee the existence of a control allowing the result to hold.  In
the feedforward inhibition result, it guarantees the existence of the
constant control $\u$ used to achieve inhibition, while in the
feedback inhibition result, it guarantees the existence of the
matrix~$\K$. The second assumption is that the dimension of the control
is at least as large as the number of task-irrelevant nodes in the
system. Intuitively, this result guarantees that the control can
inhibit every task-irrelevant node in the system (it would not be
possible to achieve this if the dimension was smaller).
% %
% \marginJC{Why? We just said in the previous sentence that it wouldb't
%   be possible for feedfoweard. Why is it possible with feedback?}
% \marginm{In the result in Erfan's first TAC paper it is seen the proof
%   doesn't require it. In Erfan's comment above (since commented out),
%   he says it is an interesting observation but we don't have any
%   further insights}
% %
% \marginJC{Push yourself a bit more! Why don't you think about an
%   explanation? What in the proof makes one thing go one way and the
%   other not? In other words, how does feedback compensate for the fact
%   that direct control may only exist for a subset of the
%   task-irrelevant nodes? }
% \marginm{I had been making mistakes reading... both require it}
% %





==> tex/simulations.tex <==
\section{Quantitative Simulations}\label{sec:simulations}


%%% Here provide the simulations on the convergence time relative to variety of parameters.

We have shown that in the hierarchical thalamocortical network we can achieve selective inhibition and recruitment under a set of conditions similar to those for the cortical network. A question of interest that remains is in the benefit of the inclusion of the thalamus in brain networks. Neuroscientific evidence exists for the thalamus allowing the cortex to effectively adjust to rapidly changing behavioural and environmental demands, along with the performance of cognitive functions such as attention and learning~\citep{RN-VK-BD-RB:14}. In this section we investigate simulations of the convergence to equilibrium in selective inhibition and recruitment for hierarchical thalamocortical networks along with their cortical counterparts to illustrate this benefit of the thalamus within our model. In particular we compare how different parameters impact the benefit of the thalamus.

We consider a variety of thalamocortical networks and the corresponding cortical network constructed by removing the connections between the thalamus and cortical regions. In these examples we consider the time it takes for the cortical regions of a network to converge to the selectively inhibited and recruited equilibrium determined by a choice of nodes to be inhibited. These examples are then focused to determine the impact of a variety of network parameters on the convergence time. 
% In particular we consider how the following parameters:


% \marginm{Once all the plots constructed choose which to keep and which to remove based on interest}

% \begin{multicols}{2}
% \begin{itemize}
%     \item Number of layers in the network
%     \item Size of each network layer
%     \item Location of the thalamus in the temporal hierarchy
%     \item Initial distance from equilibrium value
%     \item Ratio of excitatory to inhibitory nodes
% \end{itemize}
% \end{multicols}

We begin by comparing the convergence time as we vary basic system parameters, namely the number of layers in the network and the number of nodes in each network, shown in Figure~\ref{fig:convergence_speed_num_size_layers}. In each of these examples the convergence time is computed and averaged across randomly generated networks and initial conditions while varying the relevant parameters. From Figure~\ref{fig:num_layers} we can see that on average the convergence time for the thalamocortical network is shorter than for the cortical network regardless of the number of layers in the network. Meanwhile Figure~\ref{fig:layer_size} illustrates that at a given number of network layers changing the number of nodes in each layer does not have a significant impact on changing the convergence speed between the thalamocortical and cortical network.

\begin{figure}
	\centering
	\subfigure[]{
	\includegraphics[scale=0.2]{epsfiles/Convergence_Speed/num_layers.png}\label{fig:num_layers}
	}
	% \label{fig:num_layers}
	\subfigure[]{
	\includegraphics[scale=0.2]{epsfiles/Convergence_Speed/layer_size.png}\label{fig:layer_size}
	}
	% \label{fig:size_layers}
	\caption{Comparison of the convergence time for thalamocortical and cortical networks as changing the number of network layers and the size of network layers. (a) Convergence time is compared for networks with a varying number of network layers. For each number of layers $20$ networks are randomly generated and the convergence time to equilibrium is computed and averaged across these networks. The networks are composed of layers with four nodes each, split evenly between excitatory and inhibitory nodes and the initial condition is set a uniform distance from the equilibrium computed to be a fraction of the network threshold value. The thalamus is composed of four inhibitory nodes and the timescale is such that it lies in the middle of the network hierarchy. (b) Convergence time is compared for networks with a varying number of nodes in each layer. For each network layer size $10$ networks are randomly generated and the convergence time is computed and averaged. Each network is composed of $20$ layers and half of the nodes in each layer are excitatory with the remaining inhibitory. The initial condition is set a uniform distance from the equilibrium. The thalamus timescale is set such that it lies in the middle of the network hierarchy.}\label{fig:convergence_speed_num_size_layers}
\end{figure}


Now that we have seen that the thalamus can result in faster convergence to a selectively inhibited and recruited equilibrium we move on to considering thalamocortical networks with varying timescales. These are of interest due to their existence in the brain, as even when considering only the visual thalamus, there exists regions that operate at slow and fast timescales~\citep{ZY-XY-CMH-ZA-NPF-WW-SGB:17}. When varying the thalamus timescale we are considering networks in which the thalamus lies at different points in the temporal hierarchy. For a low timescale the thalamus lies lower in the network and is faster relative to more cortical regions while as the timescale increases the thalamus operates more slowly and moves higher in the network. From Figure~\ref{fig:timescale_varying} we can see that for both fast and slow thalamic timescales the convergence time of the thalamocortical network is lower than that of the strictly cortical network. What is of note is that as the timescale increases and the thalamus becomes slower the margin of improvement decreases. This can be explained by the timescale separation formed in the hierarchy by this increasing timescale. As the timescale continues to increase the thalamus begins to act as a constant relative to the cortical activity, leading to the thalamocortical network essentially becoming a cortical network with a modified constant input, which would then be expected to exhibit behaviour similar to the original cortical network.  Therefore overall it is clear that thalamic regions operating on both fast and slow timescales provide a benefit for network performance of a thalamocortical network compared to a strictly cortical network.

% \begin{figure}
% 	\centering
% 	\includegraphics[scale=0.25]{epsfiles/Convergence_Speed/timescale_varying.png}
% 	\caption{Comparison of the convergence time of thalamocortical and cortical networks with thalamic networks with varying timescales. The convergence time is computed and averaged across $30$ random networks at each thalamic timescale. Each network is composed of $20$ cortical layers of four nodes each, evenly split between excitatory and inhibitory nodes. $250$ thalamic timescales are considered uniformly spread between $0.25$ and $25$ while the cortical regions are linearly spread on the interval $[0.5,5]$. This allows for the consideration of the thalamus at all locations in the hierarchy from below all cortical layers to above. It is clear that all timescales the performance of the thalamocortical network exceeds the strictly cortical network, with the margin of improvement decreasing as the thalamic timescale increases.}\label{fig:timescale_varying}
% \end{figure}


To conclude this section we consider how the thalamus impacts networks with varying ratios of excitatory to inhibitory nodes.  There is significant evidence that inhibition in neural networks is key for selective attention~\citep{AD:13}, with strictly cortical excitatory networks lacking one of the necessary mechanisms required~\citep{ACS-MJM-MAS:16}. Due to the inhibitory nature of the thalamus, the thalamocortical network always maintains the mechanism of inhibitory control that the cortical network can lose with an increase in the proportion of excitatory nodes. As such we expect that as the proportion of excitatory nodes increases the time for convergence of the strictly cortical network will increase while the thalamocortical network will maintain better performance. Figure~\ref{fig:excitatory_ratio} matches these expectations, where we see that in networks with a low proportion of excitatory nodes the thalamocortical networks and cortical networks having essentially identical performance but as the proportion of excitatory nodes increases the thalamocortical network achieves significantly better performance. We note that as the proportion approaches having a fully excitatory network the convergence time drops dramatically, however this follows from the network converging only to zero and the upper threshold, which shortens the convergence time due to decreasing the network equilibrium value.

% \begin{figure}
% 	\centering
% 	\includegraphics[scale=0.25]{epsfiles/Convergence_Speed/frac_excitatory.png}
% 	\caption{Comparison of convergence times of thalamocortical and cortical networks with varying ratio of excitatory to inhibitory nodes. The convergence time is computed and averaged across $30$ random networks composed of $20$ layers with $20$ nodes per layer. The proportion of excitatory nodes rises from a fully inhibitory network to a fully excitatory network (with the exception of the thalamus). For inhibitory networks the performance of the thalamocortical networks and cortical networks is similar. As the number of excitatory nodes increases the performance of the thalamocortical network maintains a similar value while the cortical network is significantly worse. This changes at the high end of the spectrum when the upper bound in the dynamics limits the equilibrium value.}\label{fig:excitatory_ratio}
% \end{figure}



\begin{figure}
	\centering
	\subfigure[]{
	\includegraphics[scale=0.2]{epsfiles/Convergence_Speed/timescale_varying.png}\label{fig:timescale_varying}
	}
	% \label{fig:num_layers}
	\subfigure[]{
	\includegraphics[scale=0.2]{epsfiles/Convergence_Speed/frac_excitatory.png}\label{fig:excitatory_ratio}
	}
	% \label{fig:size_layers}
	\caption{Comparison of the convergence time of thalamocortical and cortical networks with thalamic networks with varying timescales and number of excitatory nodes. a) Convergence time is compared for networks with varying thalamic timescales. The convergence time is computed and averaged across $30$ random networks at each thalamic timescale. Each network is composed of $20$ cortical layers of four nodes each, evenly split between excitatory and inhibitory nodes. $250$ thalamic timescales are considered uniformly spread between $0.25$ and $25$ while the cortical regions are linearly spread on the interval $[0.5,5]$. This allows for the consideration of the thalamus at all locations in the hierarchy from below all cortical layers to above. It is clear that all timescales the performance of the thalamocortical network exceeds the strictly cortical network, with the margin of improvement decreasing as the thalamic timescale increases. b) Convergence time is compared for networks with varying ratio of excitatory to inhibitory nodes. The convergence time is computed and averaged across $30$ random networks composed of $20$ layers with $20$ nodes per layer. The proportion of excitatory nodes rises from a fully inhibitory network to a fully excitatory network (with the exception of the thalamus). For inhibitory networks the performance of the thalamocortical networks and cortical networks is similar. As the number of excitatory nodes increases the performance of the thalamocortical network maintains a similar value while the cortical network is significantly worse. This changes at the high end of the spectrum when the upper bound in the dynamics limits the equilibrium value.}
\end{figure}



==> tex/topologies.tex <==
\section{Brain Networks of Interconnected
  Networks}\label{sec:topologies}

Goal-driven selective attention occurs based on interactions and the
transmission of information between areas in the brain. Here, we
expand our treatment of selective inhibition and recruitment to networks composed of multiple brain regions. We maintain the model
of linear-threshold firing rate dynamics for each region and combine
them to create larger networks of networks, as described in
Box~\ref{box:construction_multi-region_networks}. GDSA can then be
studied, given its diverse functions and mechanisms, using
thalamocortical networks with multiple topologies. In particular, we
examine the following three topologies:
\begin{itemize}
\item A \emph{hierarchical cortical topology} as shown in
  Figure~\ref{fig:network_topologies}(a). In this topology, we
  consider a series of cortical regions forming a hierarchy, where
  each region is connected only to regions directly above and
  below. The resulting network of networks ignores the thalamocortical
  connections and, as such, lacks complete physical
  relevance. However, its simple setup makes it useful as a foundation
  before expanding to more complex networks and it also provides a
  baseline to understand the role of the thalamus beyond being a
  sensory relay;

\item A \emph{hierarchical thalamocortical topology} as shown in
  Figure~\ref{fig:network_topologies}(b). In this topology, the
  thalamus is a higher-order thalamic nuclei, which accepts inputs
  from cortical regions, before modulating them and transmitting the
  information to other cortical regions, forming
  transthalamic pathways parallel to the direct cortico-cortical connections. By
  connecting to each cortical region in the hierarchy, this topology
  allows for the direct connection of any two cortical regions through
  the thalamus. Such a topology appears in higher-level brain
  functions such as learning and decision-making where the thalamus
  supports the transfer of information across the prefrontal
  cortex~\citep{ASM:15};

\item A \emph{star-connected thalamocortical topology} as shown in
  Figure~\ref{fig:network_topologies}(c). In this topology, the
  thalamus node is a first-order thalamic nuclei, which transmits
  sensory or other information from subcortical structures to cortical
  regions. Here the thalamus is operating mostly as a relay, and such
  topologies arise in all sensory systems, with the exception of the
  olfactory system. Examples of first-order thalamic nuclei that
  result in this topology are the ventral posterior nucleus in the
  somatosensory system and the lateral geniculate nucleus in the
  visual system~\citep{EJR-JWG-SMS:05}.
\end{itemize}

 % \en{I think the rest of this paragraph is in fact one of the most important points of this paper, so I suggest expanding it. We can make it an itemize/enumerate environment to highlight the three-ness of the topologies discussed, and then discuss a bit more what they each mean. For example, most readers have no memory at this point of what ``For higher-order thalamic relays" even means, let alone in what biological contexts or sensory/cognitive systems the resulting topology will be useful. If we can (even briefly) address the biological contexts/phenomena/systems/... in which each of these makes most sense, that would hit a very important point. And if some (say the purely cortical one) is only for simplicity but otherwise does not have any biological relevance beyond the ones with thalamus, we can explicitly say so and briefly mention (though the details are still to come) what kinds of theoretical advantages it affords.}
  % For higher-order thalamic relays, a hierarchical thalamocortical network is formed as in Figure~\ref{fig:network_topologies}(a). In the case of first-order thalamic relays the star-connected network of Figure~\ref{fig:network_topologies}(c) is formed. Finally, GDSA can also occur in hierarchical cortical networks as in Figure~\ref{fig:network_topologies}(b). We will examine and compare conditions for selective inhibition and recruitment in each of these topologies.

% We then consider GDSA in thalamocortical networks, with two different topologies that arise in different situations. First we consider a hierarchical network in which the thalamus is operating as a higher-order relay (Figure~\ref{fig:network_topologies}(a)), before considering a star-connection thalamocortical network, where the thalamus is a first-order relay (Figure~\ref{fig:network_topologies}(c)). In addition we consider GDSA in a strictly cortical hierarchical network (Figure~\ref{fig:network_topologies}(b)) to compare with the thalamocortical networks.
% \\



\tikzset{
mynode/.style={
text width=0.06\textwidth
}}
 \begin{figure*}[htb!]
   \centering
        \subfigure[]{
     \begin{tikzpicture}
       \node[mynode, circle, draw, line width=0.6pt, minimum size = 0.1cm, inner sep=0pt] (1)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (1.north) to (1.south);
       \node[mynode, above of=1, yshift=30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (2)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (2.north) to (2.south);
       \node[mynode, below of=1, yshift=-30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (3)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (3.north) to (3.south);
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (1.90) to (2.270);
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (1.270) to (3.90);
       \node[below of=3, yshift=5pt] {$\vdots$};
       \node[above of=2, yshift=0pt] {$\vdots$};
       \node[left of=2, xshift=-20pt, yshift=10pt, scale=0.8] (i-1)
       {Subnetwork $i - 1$};
       \node[left of=1, xshift=-20pt, yshift=10pt, scale=0.8] (i) {Subnetwork $i$};
       \node[left of=3, xshift=-20pt, yshift=10pt, scale=0.8] (i+1) {Subnetwork $i +
         1$};
     \end{tikzpicture}
   }\qquad
   \subfigure[]{
     \begin{tikzpicture}
       \node[mynode, circle, draw, line width=0.6pt, inner sep=0pt] (1)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (1.north) to (1.south);
       \node[mynode, above of=1, yshift=30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (2)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (2.north) to (2.south);
       \node[mynode, below of=1, yshift=-30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (3)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (3.north) to (3.south);
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (1.90) to (2.270);
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (1.270) to (3.90);
       \node[below of=3, yshift=5pt] {$\vdots$};
       \node[above of=2, yshift=0pt] {$\vdots$};
       \node[left of=2, xshift=-20pt, yshift=10pt, scale=0.8] (i-1)
       {Subnetwork $i - 1$};
       \node[left of=1, xshift=-20pt, yshift=10pt, scale=0.8] (i) {Subnetwork $i$};
       \node[left of=3, xshift=-20pt, yshift=10pt, scale=0.8] (i+1) {Subnetwork $i +
         1$};
       \node[mynode, right of=1, xshift=30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (i-big)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       \draw[latex-latex,shorten <= 1pt,shorten >= 1pt] (1) to (i-big);
       \draw[latex-latex,shorten <= 1pt,shorten >= 1pt] (2) to (i-big);
       \draw[latex-latex,shorten <= 1pt,shorten >= 1pt] (3) to (i-big);
       \node[above of=i-big, xshift=0pt, yshift=-1pt, scale=0.8] (i1)
       {\parbox{40pt}{\centering  Thalamus}};
     \end{tikzpicture}
   }
   \qquad
   % 
   \subfigure[]{\begin{tikzpicture} \node[mynode, circle, draw, line
       width=0.6pt, inner sep=-0.3pt] (1)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (1.north) to (1.south);
       \node[above of=1, xshift = 25pt, yshift = -5pt, scale=0.8]{Thalamus};
       \node[mynode, above of=1, yshift=30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (2)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (2.north) to (2.south);
       \node[above of=2, xshift = 0pt, yshift = -5pt, scale=0.8]{Subnetwork $1$};
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (2.270) to (1.90);
       \node[mynode, left of=1, xshift=-30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (3)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (3.north) to (3.south);
       \node[below of=3, xshift = 0pt, yshift = 5pt, scale=0.8]{Subnetwork $4$};
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (3.0) to (1.180);
      
       \node[mynode, right of=1, xshift=30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (4)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (4.north) to (4.south); 
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (1.0) to (4.180);
       \node[below of=4, xshift = 0pt, yshift = 5pt, scale=0.8]{Subnetwork $2$};  
      
       \node[mynode, below of=1, yshift=-30pt, circle, draw, line
       width=0.6pt, inner sep=-0.4pt] (5)
       {\includegraphics[width=28pt]{EI_network_structure_half_inhibited}};
       % \draw[-, line width=0.3pt] (5.north) to (5.south); 
       \node[below of=5, xshift = 0pt, yshift = 0pt, scale=0.8]{Subnetwork $3$};
       \draw[latex-latex, line width=0.3pt, shorten <=1pt, shorten
       >=1pt] (5.90) to (1.270);
     \end{tikzpicture}
 }
 \caption{Topologies for brain networks considered in the paper. (a)
   multilayer hierarchical cortical network, where each network is
   only connected to the layers directly above and below it. (b)
   multilayer hierarchical thalamocortical network, where each layer
   is connected directly to the thalamus, as well as the layers
   directly above and below it. (c) star-connected thalamocortical
   network, where each cortical layer is connected to the thalamus
   layer but no direct connections exist between cortical regions.  In
   all of the plots, task-relevant excitatory and inhibitory nodes are
   depicted in red and blue, respectively, and task-irrelevant nodes
   are depicted in grey.}\label{fig:network_topologies}
 \end{figure*}

% %
% \marginJC{I don't see anything grey. Where are the task-irrelevant
%   nodes mentioned in the caption?}
%   \marginm{Changed which internal image used for clarity}
% \marginm{I have been unsuccesful in trying to get this image to stay in the text where included rather than going below the reference list.}
% % %

 \begin{myblock}{Construction of Multi-Region Brain
     Networks}\label{box:construction_multi-region_networks}
   Multi-region brain networks of networks are constructed through the
   interconnection of the dynamics of individual brain regions. This
   occurs through the definition of sensory information processing
   pathways along connections within the structure of the network. We
   recall that a single brain region, which we denote $\mathcal{N}_1$,
   is defined by the dynamics
   \begin{align*}
     \tau_1 \dot{\x}_1 &= -\x_1 + [\W_{1,1}\x_1 +
     \d_1(t)]_\zero^{\m_1}.
   \end{align*}
   With the internal dynamics of the brain region given by the
   synaptic weight matrix $\W_{1,1}$, we define the processing
   pathways between regions in the input term $\d_1(t)$. Let
   $\mathcal{N}_2$ denote a second brain region, which we assume is
   connected to $\mathcal{N}_1$, forming a network. Then, synaptic
   weight matrices $\W_{1,2}$ and $\W_{2,1}$ represent the information
   processing pathways between the two regions, defining the structure
   of the network. The input term $\d_1(t)$ for $\mathcal{N}_1$
   is then given by
   \begin{align*}
     \d_1(t) = \W_{1,2}\x_2 + \B_1\u_1(t) + \c_1,
   \end{align*}
   where $\u_1(t)$ is the control term for the region, and $\c_1$
   corresponds to any unmodeled background activity. Then, defining
   the dynamics of $\mathcal{N}_2$ with the same linear-threshold
   activation function, and defining $\d_2(t)$ analagously, the dynamics for the overall network composed
   of $\mathcal{N}_1$ and $\mathcal{N}_2$ is
   \begin{align*}
     \tau_1 \dot{\x}_1 &= -\x_1 + [\W_{1,1}\x_1 + \W_{1,2}\x_2+
     \B_1\u_1(t) + \c_1]_\zero^{\m_1}
     \\
     \tau_2 \dot{\x}_2 &= -\x_2 + [\W_{2,2}\x_2 + \W_{2,1}\x_1+
     \B_2\u_2(t) + \c_2]_\zero^{\m_2}.
   \end{align*}
   This process can then be used iteratively to construct brain
   networks of arbitrary size and connectivity structure, which we use
   to study networks with the topologies shown in
   Figure~\ref{fig:network_topologies}.
\end{myblock}

\subsection{Hierarchical Topologies}
The brain has been known to have a hierarchical organization for decades,
both in terms of structure and function~\citep{NT:50,ARL:70}. One of
these hierarchies is based upon function, in which primary sensory and
motor areas are placed at the bottom of the hierarchy, while
high-level processing areas such as the prefrontal cortex lie at the
top~\citep{DJF-DCEV:91}. Sensory information is
processed as it moves up the hierarchy, while decisions are made at
the top and information is then transmitted back down the hierarchy to perform desired
actions. It is in the top-down direction of this hierarchy that GDSA
occurs, where the higher-level layers instruct the lower layers as to
which information is relevant, thus requiring further processing for
performing the desired actions, and which should be suppressed
and prevented from further processing.
\\

In addition to being sorted based upon the direction of information
flow, a hierarchy of timescales also exists between brain regions,
which closely aligns with the former. In particular, as one moves up
the hierarchy, the regional dynamics become
slower~\citep{BG-EE-GH-AG-AK:12,UH-JC-CJH:15,SJK-JD-KJF:08}.  This
separation of timescales plays a significant role in the ability of
the network to perform selective inhibition and recruitment.
% GDSA in hierarchical topologies occurs through the layers higher in
% the network dictating the relevant information to the lower levels
% in the hierarchy.

Recall that the goal of GDSA is to have the task-irrelevant components
of the network converge to zero while the task-relevant components
converge to an equilibrium $\x^*$. In the case of a network of
networks, the determination of such equilibria at each layer is not
trivial, as the layer interconnection makes it dependent upon the
inputs of layers higher in the hierarchy. Effectively, this defines an
equilibrium map for each layer~$i$, which we denote
$h_i^1(\cdot)$. This map, given the inputs from the higher layers in
the network, returns the set of equilibria for network layer~$i$.
Fortunately, the timescale separation mentioned above simplifies
considerably the computation of these equilibrium maps. In fact, one
can set the state of the task-irrelevant nodes to zero (as this will
be taken care of by selective inhibition) and shrink the state of each
layer to strictly include the task-relevant components. The
equilibrium maps require a constant input representing the state of
the layers higher in the network, whose existence can be justified
through the timescale separation between layers in the hierarchical
network and using singular perturbation theory. Under the assumption
that the timescale separation is infinitely large, and assuming global
asymptotic stability of each layer, the state of a given layer appears
as a constant at the timescale of the lower layers in the
hierarchy. Conversely, at the timescale of layers above, the state of
a lower layer becomes a static nonlinear function of the states of the
higher layers of the hierarchy. Utilizing this, the equilibrium map
takes its inputs to be the state (modified through interconnection
matrices) of any layers higher in the network that are directly
connected (one cortical region and the thalamus in the thalamocortical
region, dependent on the location in the hierarchy). We are then able
to recursively define equilibrium maps from the bottom layer up to the
top of the hierarchy. Utilizing these equilibrium maps, and the goal
equilibrium they define for selective recruitment, we next discuss
conditions for achieving selective inhibition and recruitment in the
cortical and thalamocortical hierarchical networks.
%
% \marginJC{Somewhere above we should have a mathematical expression for
% these equilibrium maps that show the matrices $F_i$ that we use later}
% \marginm{I'm putting below for an example in the cortical hierarchy, then say it is similar in the thalamocortical but differs due to location. Gives the ability to say what is needed but leave out complicated details that can be seen in the other papers}
% %

% %
% {\color{orange}above new, below old}
% %
% As such, the desired equilibrium to be reached by any given layer in the network is based upon the inputs received from higher in the hierarchy. In order to represent this within the linear-threshold framework for GDSA, equilibrium maps are defined in a recursive fashion, such that the inputs to a layers equilibrium map come from the higher layers in the network that are directly connected. The recursive nature then iterates that the information is being passed down from the top of the hierarchy in order to dictate selective inhibition and recruitment throughout the network. These equilibrium maps are denoted by $h_i^1(\cdot)$ and define the task-relevant equilibrium values to which the task-relevant nodes can be selectively recruited for a given set of input constants. 
% \en{This paragraph gets too deep too quickly. I think we should first remind the reader what equilibrium we are talking about (from section~\ref{sec:math-def}). Then we should say what we mean by equilibrium map. The very existence of a notion like equilibrium map is justified by the timescale separation, and in fact by an infinitely large timescale separation. So we should explain that and even name-drop singular perturbation theory for those who are familiar. Here we should patiently explain the fact that at the theoretical limit of infinite timescale separations, each layer's states become constant at the timescale of the layer below and, at the timescale of the layer above, become a static nonlinear function of the above layer's states (assuming GAS of all layers). You see that there is a lot here to even explain, let alone digest for someone seeing these for the first time. And then we can talk about the recursive construction of the equilibrium maps. Somewhere within this discussion we should also remind the reader that all of this discussion is assuming that selective inhibition is perfectly assumed, so all layers are shrunk to their task-relevant parts.}
% \en{Also, essentially, what this paragraph is doing is putting together two things: the formulations in section~\ref{sec:math-def} and the timescale hierarchical structure we have just defined. So we should also explain this more clearly so that the reader appreciates the flow.}
% \\

% \en{How about moving this after the purely hierarchical case? It seems a generalization, so once this is said the hierarcihcal case becomes a bit point-less/uninteresting. But in reverse order we can present the hierarchical one first due to its simplicity, and then say this is what happens if we also have the thalamus.}


\subsubsection{Cortical Hierarchical Networks}
The cortical hierarchical network, shown in
Figure~\ref{fig:network_topologies}(a), is composed of $N$ cortical
regions each connected only to the regions directly above and
below. The cortical regions form a temporal (and functional)
hierarchy, encoded by timescales satisfying $\tau_1 \gg \tau_2 \gg
\dots \gg \tau_N$, and each region is connected only to the regions
directly above and below. We model each brain region using the
linear-threshold firing rate model
in~\eqref{eq:full_lin_thresh_dynamics_for_selective_inhibition},
resulting in the network dynamics
\begin{align}\label{eq:cortical_hierarchy_dynamics}
  \tau_i\dot{\x}_i &= -\x_i + [\W_{i,i}\x_i(t) + \W_{i,i-1}\x_{i-1}(t)
  + \W_{i,i+1}\x_{i+1}(t) + \B_i\u_i(t) + \c_i]_\zero^{\m_i}, \notag
  \\
\end{align}
for $i \in \until{N}$. This dynamics then leads to the equilibrium map for a layer in the cortical hierarchy taking the following form
\begin{align}\label{eq:cortical_hierarchy_equilibrium_map}
  h_i^1(\c) = \{\x_i^1 ~|~ \x_i^1 = [\W_{i,i+1}^{11}h_{i+1}^1(\W_{i+1,i}^{11}\x_i^1 + \c_{i+1}^1) + \W_{i,i}^{11}\x_i^1 + \c]_\zero^{\m_i} \}.
\end{align}
{\color{blue}From this dynamics we can define equilibrium maps for each layer in the cortical hierarchy, each giving the set of possible equilibrium points. Due to the interconnected form of the dynamics the maps are defined recursively as follows. For the bottom layer of the network the equilibrium map is defined as
\begin{align}
  h_N^1(\c) = \{\x_N^1 ~|~ \x_N^1 = [\W_{N,N}^{11}\x_N^1 + c]_\zero^{\m_N} \}.
  \end{align}
Then for layers $i \until{N-1}$ the equilibrium maps are defined as
\begin{align}
  h_i^1(\c) = \{\x_i^1 ~|~ \x_i^1 = [\W_{i,i+1}^{11}h_{i+1}^1(\W_{i+1,i}^{11}\x_i^1 + \c_{i+1}^1) + \W_{i,i}^{11}\x_i^1 + \c]_\zero^{\m_i} \}.
\end{align}
}

These maps can also be written in a switched-affine form, denoted by $h_i^1(\c) = \F_{\lambda} \c + \f_{\lambda}$ (details on this form can be found in~\cite{EN-JC:21-tacII}). This representation of the equilibrium map gives rise to a gain matrix $\bar{\F}_i$, which is defined as the entry-wise maximum of the matrix $|\F_{\lambda}|$ over all of the switching regions. These gain matrices play a role in the following result which provides conditions upon the structure of the network such that GDSA
is achieved.

% \en{I think this discussion is another reason for bringing the purely cortical one first. Now we are saying the general case first, then brining a special case and even saying that it's not quite realistic. So why bother? I think it's value is laying down the foundation for the thalamocortical version. I would also remove the next couple of sentences because it doesn't make sense to study something just to compare it with something else. We will compare everything later, but now we should say why each network has a merit in its own, otherwise its comparison with the thalamcortical network becomes pointless as well.}

\begin{theorem}\longthmtitle{Selective Inhibition and Recruitment in
    Hierarchical Cortical Networks}\label{thrm:cortical_conditions}
  Consider a cortical hierarchical network governed by a
  linear-threshold dynamics and suppose subnetwork $\mathcal{N}_1$ has
  bounded trajectories. If
  \begin{align*}
    \rho(|\W_{i,i}^{11}| +
    |\W_{i,i+1}^{11}|\bar{\F}_{i+1}|\W_{i+1,i}^{11}|) < 1, \qquad
    \forall i \in \until{N},
  \end{align*}
  % % 
  % \marginJC{Where did we explain what $\bar{\F}_{i+1}$ stand for?}
  % % 
  then there exists $\K_i$ and $\bar{\u}_i(t)$ such that using the
  feedback-feedforward control $\u(t) = \K_i\x_i(t) + \bar{\u}_i(t)$,
  for all $i$, gives
  \begin{align*}
    \begin{cases}
      \x_i^0(t) \to \zero & \mathrm{(Selective~Inhibition)}
      \\
      \x_i^1(t) \to h_i^1(\W_{i,i-1}^{11}\x_{i-1}^1(t) + \c_i^1) &
      \mathrm{(Selective~Recruitment)}
    \end{cases}
  \end{align*}
  as the timescales satisfy $\frac{\tau_i}{\tau_{i-1}} \to 0$ for all $i \in \{2,\dots,N\}$.
\end{theorem}

This result can be interpreted as follows. The condition involving the
spectral radius at each layer involves two terms: the internal
dynamics of layer $\mathcal{N}_i$ and the impact of its
interconnection with $\mathcal{N}_{i+1}$. Due to the timescale
separation between the layers in the hierarchy, the connection from
$\mathcal{N}_{i+1}$ acts as a static nonlinearity. Thus the sum
combines the two pathways that $\mathcal{N}_i$ has to impact its
state, and the spectral radius provides a conservative upper bound on
the combined effects of these pathways. Then, if the spectral radius
conditions hold, reduced-order dynamics for the task-relevant
components in the network constructed by replacing connections from
lower layers with their equilibrium values are GES~\citep[Theorem
IV.4]{EN-JC:21-tacII}, which allows for convergence to the desired
equilibrium for GDSA. The result $\x_i^0(t) \to \zero$ shows the
task-irrelevant components of the dynamics converging to zero, while
$\x_i^1(t) \to h_i^1(\W_{i,i-1}^{11}\x_{i-1}^1(t) + \c_i^1)$ gives the
convergence of layer $\mathcal{N}_i$ to an equilibrium, which we see
is dependent on inputs from higher in the hierarchy, as expected.
% \marginm{Personally, I think the theorem environment here is reasonable - having one for each of the topologies. However, if desired this could be replaced with an explanation saying that it is achieved by having the conditions for the thalamocortical hold with all thalamocortical connections equaling zero. I will wait for your thoughts on this}
% \en{I agree. I would just spend some time discussing the assumption and conclusions of the theorem in plain English. We have worked with these long enough that they are clear, but for a layer reader they are extremtly notation-heavy and confusing. Even if repetative, I would explain what the spectral radius condition says (in particular the meaning of the two terms in it: the direct internal connections of layer i plus the indirect connections through layer i+1 that is acting as a static nonlinearity due to timescale separation, so each state of layer i has two pathways for affecting any other state of layer i and this is a conservative upper bound on the combined effects of these two pathways) as well as how one should intuitively read each of $\x_i^0(t) \to \zero$ and $\x_i^1(t) \to h_i^1(\W_{i,i-1}^{11}\x_{i-1}^1(t) + \c_i^1)$.}

We now give some intuition on the gain matrices $\bar{\F}_i$.
% %
% \marginJC{This red part should be earlier, probably when discussing
%   the equilibrium maps, otherwise the theorem statement is hanging
%   with incomplete meaning when we actually state it}
% %
 They provide a worst-case bound on how much the equilibrium
point of a layer $\mathcal{N}_i$ can change based on one unit of
change in the state of layer $\mathcal{N}_{i-1}$, and as such its use
in the spectral radius conditions covering pathways for modifying
system states makes the bound conservative.  Further, the final
condition $\tau_{i}/\tau_{i-1} \to 0$ corresponds to the timescale
separation between layers becoming infinitely large. This separation,
creating completely distinct timescales between each layer, provides
the base for being able to apply a singular perturbation argument to
prove the result. It is important to note that, while the result calls
for an infinite timescale separation, in brain pathways the timescale
ratios between successive layers is between $1/1.5$ and $1/2.5$, which
is typically more than enough to selectively inhibit and recruit the
system succesfully with a small degree of tracking
error~\citep{EN-JC:21-tacII}.

\subsubsection{Thalamocortical Hierarchical
  Networks}\label{sec:thalamocortical_hierarchy}
The thalamocortical hierarchical network, shown in
Figure~\ref{fig:network_topologies}(b), is composed of $N$ cortical
regions, each connected only to the regions directly above and below,
along with an additional thalamic region that connects to all of the
cortical regions. While the thalamus is actually composed of more than
one region, we simplify the model by assuming all thalamic nuclei
relevant to the network are contained in the single thalamic
subnetwork. The cortical regions form the same temporal (and
functional) hierarchy, but now the thalamus, which forms parallel
transthalamic pathways between the cortical regions, also lies within
the hierarchy. The exact position of the thalamus within the timescale
is dependent upon which cortical regions belong in the network, but it
can lie at any
point~\citep{JAH-SM-KEH-JDW-HC-AB-PB-SC-LC-AC:19}. Without loss of
generality we assume that the thalamus lies at a point in the middle
of the hierarchy, with $\tau_a \gg \tau_T \gg \tau_b$ for some $a,b
\in \until{N}$ with $b = a+1$. All of the results to follow are valid
regardless of the location of the thalamus, with only slight changes
in the resulting expressions.
\\

In this network, the thalamus is operating as a higher-order relay,
indicated by having cortical inputs and forming transthalamic pathways
between cortical regions~\citep{SMS:12}. As before, we model each brain
region using a linear-threshold firing rate
model~\eqref{eq:full_lin_thresh_dynamics_for_selective_inhibition},
giving the following dynamics for the full $N$-layer hierarchical
network.
\begin{align}\label{eq:thalamocortical_hierarchy_dynamics}
  \tau_i\dot{\x}_i &= -\x_i + [\W_{i,i}\x_i(t) + \W_{i,i-1}\x_{i-1}(t)
  + \W_{i,i+1}\x_{i+1}(t) + \W_{i,T}\x_T(t) + \B_i\u_i(t) +
  \c_i]_\zero^{\m_i} \notag
  \\
  \tau_T\dot{\x}_T &= -\x_T + [\W_{T}\x_T + \sum_{i=1}^N \W_{T,i}\x_i
  + \B_T\u_T(t) + \c_T]_\zero^{\m_T},
\end{align}
where $i \in \until{N}$. We note that the dynamics are similar to
those of the cortical hierarchical network, but the addition of the
thalamus enriches the dynamics of each individual layer due to the
additional network connections. As a hierarchical network, equilibrium maps are defined in a recursive fashion, however, the changes to the dynamics from the thalamus result in the structure of the equilibrium maps changing depending upon the location of the corresponding layer in the network. Despite this difference, equilibrium maps still have a switched-affine representation and as such corresponding gain matrices $\bar{\F}_i$, but the values will differ from a cortical network with the same cortico-cortical connections due to the thalamic influence.

The following result now connects the
structure of all network layers in the hierarchical thalamocortical network to the desired behaviors under GDSA.
%We now provide a result on selective inhibition and recruitment in
%thalamocortical networks.
% %
% \marginJC{Shouldnt' we comment on what happens to the equilibrium maps
% before we get into the result? In particular, what do the $\bar{F}_i$
% denote? Since we're using the same notation, the reader will
% understandably assume they are the same matrices as before, whereas I
% doubt that's the case.}
% %

\begin{theorem}\longthmtitle{Selective Inhibition and Recruitment in
    Hierarchical Thalamocortical
    Networks}\label{thrm:thalamocortical_hierarchy_conditions} 
  Consider a thalamocortical hierarchical network governed by a
  linear-threshold dynamics and suppose subnetwork $\mathcal{N}_1$ has
  bounded trajectories. If
  \begin{align*}
    \rho(|\W_{i,i}^{11}| +
    |\W_{i,i+1}^{11}|\bar{\F}_{i+1}|\W_{i+1,i}^{11}|) < 1,
  \end{align*}
  for layers below the thalamus,
    \begin{align*}
      \rho(|\W_{i,i}^{11}| +
      |\W_{i,i+1}^{11}|\bar{\F}_{i+1}|\W_{i+1,i}^{11}| +
      |\W_{i,T}^{11}|\bar{\F}_T|\W_T^{11}|) < 1,
  \end{align*}
  for layers above the thalamus, and
  \begin{align*}
    \rho(|\W_{T}^{11} + \sum_{i=b}^N |\W_{T,i}^{11}|\bar{\F}_i|\W_{i,i}^{11}|) < 1,
  \end{align*}
  then there exists $\K_i$ and $\bar{\u}_i(t)$ such that using the
  feedback-feedforward control $\u(t) = \K_i\x_i(t) + \bar{\u}_i(t)$,
  for all $i$, gives
  \begin{align*}
      \begin{cases}
        \x_i^0(t) \to \zero & \forall i \in \{2,\dots,N,T\}
        \\
        \x_i^1(t) \to h_i^1(\W_{i,i-1}^{11}\x_{i-1}^1(t) + \c_i^1) &
        \mathrm{for~layers~above~the~thalamus}
        \\
        \x_i^1(t) \to h_i^1(\W_{i,i-1}^{11}\x_{i-1}^1(t) +
        \W_{i,T}^{11}\x_T^1(t) + \c_i^1) & \mathrm{
          for~layers~below~the~thalamus}
        \\
        \x_T^1(t) \to h_T(\sum_{i=1}^a \W_{T,i}^{11}\x_i^1(t) + \c_T).
        & \mathrm{ for~the~thalamus}
  \end{cases}
  \end{align*}
  as the timescales satisfy $\frac{\tau_i}{\tau_{i-1}} \to 0$ and
  $\frac{\tau_T}{\tau_b} \to 0$ for all $i \in \{2,\dots,N\}$.
\end{theorem}

\marginm{Example here - I also want to have comparison with star-connected as safety net}
Note the similarity with the conditions for GDSA in the cortical
hierarchy given in Theorem~\ref{thrm:cortical_conditions}.  The
results are dependent on conditions utilizing the spectral radius to
give a bound on the ability of the internal dynamics and
interconnections to impact the state of network layers. The conditions
in this result however include the interconnections between the
thalamus and the cortical regions, which provide an additional pathway
for impacting the dynamics. Assuming these connections are satisfied
to guarantee stable reduced-order dynamics, the result guarantees
selective recruitment to a unique equilibrium as the timescale ratio
approaches zero, giving separation between the network layers. This
equilibria is defined based upon the equilibrium maps for each layer.
However, the presence of the thalamus modifies the details of these
maps depending on their location in the hierarchy, which is reflected by the equilibrium maps $h_i^1(\cdot)$ for each layer taking different inputs dependent on the layer's location in the hierarchy.
% %
% \marginJC{Not sure what we want to convey here: what does ``we
%   distinguish the convergence'' mean?}
% %
We further compare these results in Section~\ref{sec:discussion}.

% Here the terms $\bar{\F}_i$ represent gain matrices based upon a
% switched-affine representation of the equilibrium maps. This result
% is based upon a singular perturbation argument, and we can see that
% the separation of timescales, forming the hierarchy is key for
% allowing selective inhibition and recruitment.  \en{I think both of
% these sentences need more explanation. First, what's an intuition
% for $\bar{\F}_i$? Gain in what sense (gain from what to what)? It's
% essentially a conservative upper bound on the largest input-output
% gain of the equilibrium map of layer $i$ (or $i+1$?) over the entire
% state space, i.e., the worst case bound on how much the equilibrium
% point of the $i$'th layer can change for one unit change in the
% states of layer $i-1$ (or something like that). Then, the link to
% singular perturbation theory can also be expanded a little bit I
% think.}

\subsection{Star-Connected Thalamocortical Networks}
% A star-connected network, as shown in
% Figure~\ref{fig:network_topologies}(c), arises when the thalamus
% operates as a relay center, with an input signal (typically from a
% subcortical source) being sent to multiple distinct cortical
% regions. As the cortical regions in this network are not directly
% related, there is no temporal timescale formed. For this reason, the
% singular perturbation methods used for hierarchical structures are no
% longer applicable. We examine this interconnection structure as it
% arises frequently, particularly in networks that process sensory
% information.

% We assume the thalamic region being modeled is a first-order relay,
%  % \en{What does a first-order relay mean? one-step/one-hop?}
% relaying a subcortical sensory input signal to multiple cortical
% regions~\citep{SMS:12} and we assume one of the non-thalamic
% subnetworks in the star-connected network is a subcortical structure
% providing that input signal.  We model this region with a
% linear-threshold firing rate model in the same manner as the other
% regions in the network, except that it includes no explicit control
% term, as we do not manipulate the input signal that is determined by
% sensory input to the body.
% % \en{What does having no independent control term mean? And why do we
% % do this? What's the biological meaning and justificaiton of it?}.
% Accordingly, the dynamics for a star-connected thalamocortical network
% with $N-1$ cortical regions is given by
% \begin{align}\label{eq:star_connected_dynamics}
%   \tau_1\dot{\x}_1 &= -\x_1 + [\W_{1,1}\x_1 + \W_{1,T}\x_T +
%   \c_1]_\zero^{\m_1} \notag 
%   \\ 
%   \tau_i \dot{\x}_i &= -\x_i + [\W_{i,i}\x_i + \W_{i,T}\x_T + \B_i\u_i
%   + \c_i]_\zero^{\m_i} \notag 
%   \\
%   \tau_T\dot{\x}_T &= -\x_T + [\W_{T}\x_T + \sum_{i=1}^N \W_{T,i}\x_i
%   + \B_T\u_T + \c_T]_\zero^{\m_T},
% \end{align}
% where $i \in \{2,\dots,N\}$ and $\x_1$ denotes the states of the
% subcortical region providing sensory input to the thalamus.

% When considering the selective inhibition and recruitment in
% star-connected networks, we examine two different network states.
% % %
% % \marginJC{This makes it sound like we're gonna treat both cases
% %   equally, but we only have 1 theorem. I wonder if we could just
% %   present one result (the feedback one) and then instead say that when
% %   the interconnection is zero, this is actually a cascaded system
% %   (since this is really a particular case).}
% % %
% In addition to considering a general star-connected network, we discuss a cascade system, in which there is no feedback from the cortical regions to the thalamus, nor from the thalamus to the
% input region. The cascade system forms a basis for the operation of the thalamus as
% a first-order relay, as it is transmitting information from a
% subcortical source to cortical regions. We then extend on the cascade system to the scenario in which feedback exists between the brain regions. 

% \begin{theorem}\longthmtitle{Selective Inhibition in a
%     Star-Connected Network~\citep{MM-JC:22}}\label{thrm:star_network}
%   Consider a star-connected thalamocortical network with $N-1$
%   cortical regions, denoted $\mathcal{N}_2,\dots,\mathcal{N}_N$, and a
%   subcortical input layer, $\mathcal{N}_1$, governed by the
%   dynamics~\eqref{eq:star_connected_dynamics}. Suppose the following hold for all values of $\c_i$, $i \in \until{N}$, and $\c_T$:
%   \begin{enumerate}
%      \item The input layer, $\mathcal{N}_1$, has no nodes to be inhibited and the dynamics
%      \begin{align*}
%        \tau_1\dot{\x}_1 = -\x_1 + [\W_{1,1}\x_1 + \c_1]_\zero^{\m_1},
%      \end{align*}
%      is GES to a unique equilibrium for all constants $\c_1$. Further,
%      assume $\W_{1,1} \in \mathcal{L}$.
%      \item For $i \in \{2,\dots,N,T\}$, the matrix $\W_{i,i}^{11} \in \mathcal{L}$.
%      \item The interconnection matrices $\W_{i,T}$ and $\W_{T,i}$, $i \in \until{N}$, are small enough such that the matrix
%      \begin{align*}
%        \bar{\W}^{11} = \begin{bmatrix}
%          \W_{1,1} & \zero & \dots & \zero & \W_{1,T}^{11} \\
%          \zero & \W_{2,2}^{11} & \dots & \zero & \W_{2,T}^{11} \\
%          \vdots & \vdots & \ddots & \vdots & \vdots \\
%          \zero & \zero & \dots & \W_{N,N}^{11} & \W^{11}_{N,T} \\
%          \W_{T,1}^{11} & \W_{T,2}^{11} & \dots & \W_{T,N}^{11} & \W_T^{11}
%        \end{bmatrix},
%      \end{align*}
%      is totally $\mathcal{L}$-stable.
%    \end{enumerate} 
%    Then the cortical layers $\mathcal{N}_i$, $i \in \{2,\dots,N\}$,
%    can be selectively inhibited and recruited to a unique equilibrium.
% \end{theorem}

% First, we note that we have a cascade system when $\W_{1,T} = \zero$ and $\W_{T,i} = \zero$ for $i \in \{2,\dots,N\}$. In this case we have that the third condition in Theorem~\ref{thrm:star_network} becomes trivially satisfied and the ability to selectively inhibit and
% recruit the nodes in the star-connected cascade thalamocortical
% network is dependent solely on the internal dynamics of the
% task-relevant component of each layer, rather than the synaptic
% weights of the connection between the thalamus and the cortical
% regions.
% % \en{Apart from some grammatical revision that the next sentence needs, I will be much more careful in stating these from neuroscience. In fact, it is quite commonly believed that feedback connections are stronger than feedforward connections in early sensory stages. If I remember correctly, V1 projects to LGN 10 times more than LGN does to V1. We can still mention the synergies between your theoretical small-feedback results and the neuroscience observations you list, but should use very careful and humble wording.}
% While this result establishes that it is possible to selectively
% inhibit and recruit networks without feedback, this is an unrealistic
% assumption as feedback does exist within the brain. This result establishes that selective inhibition and
% recruitment is possible in systems with feedback, provided that the
% magnitude of the interconnections between the thalamus and cortical regions is sufficiently small. Though restrictive, this does
% align with some neuroscientific observations. In particular, this
% result, which establishes a bound upon the amount of corticothalamic
% feedback (the magnitude of the bound is dependent upon the
% thalamocortical connections) aligns with the fact that it has been observed that high amounts
% of corticothalamic feedback can result in pathological
% behaviour~\citep{KG-JMD:20}. In particular, strong corticothalamic
% feedback has been found to coincide with epileptic loss of
% consciousness in absence seizures due to over-inhibition of the
% cortical regions~\citep{GKK:01}.

%%%%%%%%%%%%%%%% UPDATES AS PER BASE PAPER

{\color{blue}
A star-connected network, as shown in
Figure~\ref{fig:network_topologies}(c), arises when the thalamus
operates as a relay center, with an input signal (typically from a
subcortical source) being sent to multiple distinct cortical
regions. As the cortical regions in this network are not directly
related, there is no temporal timescale formed.
%  For this reason, the
% singular perturbation methods used for hierarchical structures are no
% longer applicable. 
We examine this interconnection structure as it
arises frequently, particularly in networks that process sensory
information.

We assume the thalamic region being modeled is a first-order relay,
 % \en{What does a first-order relay mean? one-step/one-hop?}
relaying a subcortical sensory input signal to multiple cortical
regions~\citep{SMS:12} and that one of the non-thalamic
subnetworks in the star-connected network is a subcortical structure
providing that input signal.  We model this region with a
linear-threshold firing rate model in the same manner as the other
regions in the network, except rather than an explicit control
term the sensory input to the subcortical structure is represented by a time-varying input signal, $\c_1(t)$.
Accordingly, the dynamics for a star-connected thalamocortical network
with $N-1$ cortical regions is given by
\begin{align}\label{eq:star_connected_dynamics}
  \tau_1\dot{\x}_1 &= -\x_1 + [\W_{1,1}\x_1 + \W_{1,T}\x_T +
  \c_1(t)]_\zero^{\m_1} \notag 
  \\ 
  \tau_i \dot{\x}_i &= -\x_i + [\W_{i,i}\x_i + \W_{i,T}\x_T + \B_i\u_i
  + \c_i]_\zero^{\m_i} \notag 
  \\
  \tau_T\dot{\x}_T &= -\x_T + [\W_{T}\x_T + \sum_{i=1}^N \W_{T,i}\x_i
  + \B_T\u_T + \c_T]_\zero^{\m_T},
\end{align}
where $i \in \{2,\dots,N\}$ and $\x_1$ denotes the states of the
subcortical region providing sensory input to the thalamus.

Due to the lack of temporal hierarchy in this network topology the singular perturbation methods used when considering the hierarchical networks no longer apply. First, with the lack of timescale separation, the equilibrium of the network is no longer determined through recursive equilibrium maps and instead must be computed concurrently for all network layers. In particular the network equilibrium is given by the solution to the following set of nonlinear equations
\begin{align*}
  % \x_1^1 &= [\W_{1,1}^{1,\all}\x_1 + \W_{1,T}^{1,\all}\x_T +
  % \c_1^1 ]_\zero^{\m_1^1} \notag
  % \\
  \x_i^1 &= [\W_{i,i}^{1,\all}\x_i + \W_{i,T}^{1,\all}\x_T +
  \c_i^1]_\zero^{\m_i^1}, \qquad i = 1,\dots,N, \notag 
  \\
  \x_T^1 &= [\W_T\x_T + \sum_{i=1}^N \W_{T,i}\x_i +
  \c_T^1]_0^{\m_T^1}.
\end{align*}

For considering selective inhibition and recruitment in the star-connected topology we instead use results on the stability slowly varying nonlinear systems, which is dependent on having the input signal to the subcortical region, $\c_1(t)$, having a bounded rate derivative. In addition, we allow for a slightly weaker notion of selective inhibition and recruitment in which the convergence to zero and the equilibrium, respectively, is within a constant $\epsilon$. The following result provides conditions such that the thalamocortical network with a star-connected topology can achieve this notion of selective inhibition and recruitment.



\begin{theorem}\label{thrm:star_connected}
  Consider an $N$-layer star-connected thalamocortical network with $N-1$ cortical regions $\mathcal{N}_2,\dots,\mathcal{N}_N$, thalamic layer $\mathcal{N}_T$ and subcortical input layer $\mathcal{N}_1$. Suppose the following hold for all values of $\c_i \in \R^{n_i}$, $i \in \{2,\dots,N\}$ and $\c_T \in \R^{n_T}$:
  \begin{enumerate}
    \item The input layer $\mathcal{N}_1$ has no nodes to be inhibited, $\rho(\W_{1,1}|) < 1$, and the input $\c_1(t)$ lies in a compact set and has a bounded rate derivative;
    \item For each $i \in \{2,\dots,N\}\cup\{T\}$, the matrix $\W_{i,i}^{11}$ satisfies $\rho(|\W_{i,i}^{11}) < \alpha_i$, with $\alpha_i < 1$;
    \item If $\rho(\sum_{i=1}^N|\W_{i,T}^{11}\W_{T,i}^{11}|) \neq 0$, then the matrix of task-relevant interconnections
    \begin{align*}
        \bar{\W}^{11} &= \begin{bmatrix}
    \W_{1,1} & \zero & \dots & \zero & \W_{1,T}^{11} \\
    \zero & \W_{2,2}^{11} & \dots & \zero & \W_{2,T}^{11} \\
    \vdots & \dots & \ddots & \vdots & \vdots \\
    \zero & \zero & \dots & \W_{N,N}^{11} & \W_{N,T}^{11} \\
    \W_{T,1}^{11} & \W_{T,2}^{11} & \dots & \W_{T,N}^{11} &
    \W_{T}^{11}
  \end{bmatrix},
    \end{align*}
    with Schur decomposition\footnote{For a matrix $\W$ we consider the Schur decomposition $\W = \mathbf{Q}^\top(\mathbf{D}+\mathbf{N})\mathbf{Q}$ where $\mathbf{Q}$ is unitary,
$\mathbf{D}$ is diagonal, and
$\mathbf{N}$ is upper triangular with a zero
diagonal~\citep{KEC:86}.} $\bar{\W}^{11} = \mathbf{Q}^\top(\mathbf{D}_{\bar{\W}^{11}} +
\mathbf{N}_{\bar{\W}^{11}})\mathbf{Q}$, is such $\alpha + \max(\delta,\delta^{1/p}) < 1$, where $p$ is the dimension of $N_{\bar{\W}^{11}}$ and
    \begin{align*}
      \alpha &= \max_{i \in \{2,\dots,N\}\cup\{T\}}\{\alpha_i\}, \qquad \delta = \gamma \sum_{j=1}^{p-1}\norm{N_{\bar{\W}^{11}}}^j \\
      \gamma &= \max\{\sum_{i=1}^{N-1}\W_{i,t}^{11}\W_{i,T}^{11^\top}, \sum_{i=1}^{N-1}\W_{T,i}^{11}\W_{T,i}^{11^\top} \}
    \end{align*}
  \end{enumerate}
  Then there exists equilibrium trajectories $\x_i^*$ and $\epsilon > 0$ such that
  \begin{align*}
      \begin{cases}
        \lim_{t \to \infty}\norm{\x_1(t) - \x_1^*(\c_1(t))} < \epsilon & \mathrm{(Selective~Recruitment~of~Driving~Layer)}
        \\
        \intertext{and for all layers $\{\mathcal{N}_i\}_{i=2}^{N}$ and
      $\mathcal{N}_T$,}   \quad \lim_{t \to
      \infty} \norm{\x_i^0(t)} < \epsilon; & \mathrm{(Selective~Inhibition)}
    \\
     \quad \lim_{t \to \infty} \norm{\x_i^1(t)
      - \x_i^{1^*}(\c_1(t),\dots,\c_N,\c_T)} < \epsilon & \mathrm{(Selective~Recruitment)}
  \end{cases}
  \end{align*}
  Further, if $\norm{\dot{\c}_1(t)} \to 0$ then $\epsilon = 0$.
\end{theorem}

Theorem~\ref{thrm:star_connected} can be interpreted as the star-connected network can achieve selective inhibition and recruitment if each layer of the network dynamics is independently stable and the magnitude of the thalamocortical and corticothalamic connections does not exceed a determined stability margin. This bound on the magnitude of the corticothalamic feedback in the network aligns with neuroscientific observations: it has been seen that enhanced corticothalamic feedback can result in pathological behaviour~\citep{KG-JMD:20}. In particular, strong corticothalamic
feedback has been found to coincide with epileptic loss of
consciousness in absence seizures due to over-inhibition of the
cortical regions~\citep{GKK:01}.

\marginm{Not sure about keeping this on cascade}
Another form of a star-connected system that is of theoretical
interest is a cascade network. In this network there exists no
feedback from the thalamus to the driving region, nor from the
cortical regions to the thalamus. This is reflected by
the interconnection matrices $\W_{1,T}$ and $\W_{T,i}$ being equal to zero for all $i \in
\{2,\dots,N\}$. While not fully biologically accurate, as the
corticothalamic feedback connections do exist in the
brain~\cite{KG-JMD:20}, this network encodes the most basic concept of
a relay station for the thalamus. We note that, since
$\W_{i,T}\W_{T,i} = \zero$ for all $i \in \{1,\dots,N\}$, the
assumption~(iii) of Theorem~\ref{thrm:star_connected} is not
needed. As such, the structural requirements for achieving selective
inhibition and recruitment reduce to only being upon the internal
dynamics of each layer (cf. assumption~(ii) of
Theorem~\ref{thrm:star_connected}), which in fact can be
loosened to $\rho(\W_{ii}^{11}) < 1$, as a stability margin is no
longer required. Therefore, in contrast to both hierarchical networks
and star-connected networks with feedback, for a cascade
star-connected network, selective inhibition and recruitment has no
dependence on the magnitude of the interconnections, and is instead
dependent only on the internal layer dynamics along with the input
signal.
}










%%%%%%%%%%%%%%%%
\subsection{Star-Connected Topology as a Safety Net for a Hierarchical Thalamocortical Network}
A star-connected thalamocortical network can arise in the brain in
cases outside of the thalamus' role as a sensory relay. If a
hierarchical thalamocortical network incurs injury such that one or
more of the information pathways between cortical regions are damaged,
the network topology becomes locally akin to the star topology of
Figure~\ref{fig:network_topologies}(c). In the case of a strictly
cortical network, on the other hand, injuries separating cortical
regions would completely hamper the flow of information, including the network's ability for selective inhibitition
and recruitment. This distinction underscores an important role played
by the parallel transthalamic connections between cortical regions in
increasing redundancy (and therefore robustness) and maintaining
information transfer and the possibility for selective inhibition and
recruitment despite cortico-cortical disconnections due to
injury~\citep{MM-JC:22}. In this way, the star-connected
topology acts as a safety net for the thalamocortical network,
allowing the function to persist despite damage.
\marginm{Example comparing with standard}
\begin{myblock}{Remote Synchronization in Star-Connected
    Thalamocortical Networks}
  A phenomenon of vast classical and recent interest in neuroscience
  is that of synchronization between brain
  regions~\citep{SRC-BV:17,GB-AD:04}. In particular, \emph{remote
    synchronization} refers to the condition where regions in a
  network synchronize despite a lack of direct links between
  them~\citep{LVG-AC-AF-LF-JG-MF:13}. Remote synchronization is
  frequently studied in networks of oscillators, such as the Kuramoto
  model~\citep{HS-YK:86} of neural population phase oscillators. In
  particular, \cite{YQ:19} studies remote synchronization in
  star-connected networks where synchronization can only happen
  remotely between peripheral nodes due to the lack of direct
  connections between them.

  % Another occurrence frequently studied within the brain is the
  % presence of
  % oscillations~\cite{EN-JC:19-acc,SRC-BV:17,GB-AD:04}. In~\cite{YQ:19}
  % the authors model neuronal populations with Kuramoto
  % oscillators~\cite{HS-YK:86} and they examine the phenomenon of
  % \emph{remote synchronization}. Remote synchronization occurs in a
  % network where oscillators synchronize despite no direct
  % connections or sequence of synchronized oscillators between
  % them~\cite{LVG-AC-AF-LF-JG-MF:13}. Given the lack of direct
  % connections, the star-connected topology arises when considering
  % this phenomenon.

  Remote synchronization is also commonly observed in the brain
  between distant cortical regions, often in the context of functional
  connectivity analysis~\citep{VV-PH:14}. Given the thalamus' star-like
  connectivity to cortical regions, it has been suggested to play a
  key role in remote synchronization within the
  brain~\citep{LG-CM-AV:10}. Interestingly, it is shown
  in~\cite{VN-MV-MC-ADG-VL:13} that remote synchronization is
  dependent on symmetry between the outer regions in a star-connected
  topology, a phenomenon that is also shown to hold for remote
  synchronization of both linear-threshold and Kuramoto oscillator
  star-connected thalamocortical networks in~\cite{MM-JC:22}
  and~\cite{YQ:19}, respectively.
\end{myblock}

% %
% \marginJC{I like the text in the block, but it seems to be missing the
% connection with what we've discussed in the main body. How should the
% reader connect selective recruitment and inhibition with remote
% synchronization? Or is it at the level of structural conditions? }
% \marginm{More at the structural level - conditions are mainly dependent on dynamics of individual layers similarly to selective inhibition in star. In addition the original point was showing a further application of this network model}
% %



